Randomized Nystr\"om approximation of non-negative self-adjoint operators

The randomized singular value decomposition (SVD) has become a popular approach to computing cheap, yet accurate, low-rank approximations to matrices due to its efficiency and strong theoretical guarantees. Recent work by Boull\'e and Townsend (FoCM, 2023) presents an infinite-dimensional analog of the randomized SVD to approximate Hilbert-Schmidt operators. However, many applications involve computing low-rank approximations to symmetric positive semi-definite matrices. In this setting, it is well-established that the randomized Nystr\"om approximation is usually preferred over the randomized SVD. This paper explores an infinite-dimensional analog of the Nystr\"om approximation to compute low-rank approximations to non-negative self-adjoint trace-class operators. We present an analysis of the method and, along the way, improve the existing infinite-dimensional bounds for the randomized SVD. Our analysis yields bounds on the expected value and tail bounds for the Nystr\"om approximation error in the operator, trace, and Hilbert-Schmidt norms. Numerical experiments on integral operators arising from Gaussian process sampling and Bayesian inverse problems are used to validate the proposed infinite-dimensional Nystr\"om algorithm.

==> Notes/finitedim_gnystrom.tex <==
\section{Finite dimensional generalized Nyström}
Let $\bm{A} \in \mathbb{R}^{m \times n}$, and $\bm{\Omega} \sim N(\bm{0},\bm{K})$ be $n \times (k + p)$, and $\bm{\Psi} \sim N(\bm{0},\bm{S})$ be $m \times (k + p + \ell)$. Define the generalized Nyström approximation as $\widetilde{\bm{A}} = \bm{A\Omega} (\bm{\Psi}^T\bm{A\Omega})^{\dagger} \bm{\Psi}^T \bm{A}$. Let $\bm{Q}\bm{R} = \bm{A}\bm{\Omega}$ be the QR-decomposition of $\bm{A\Omega}$. Let $\bm{Q}_{\bot}$ be an orthonormal basis for the orthogonal complement of $\range(\bm{Q})$. Then $\widetilde{\bm{A}} = \bm{Q}(\bm{\Psi}^T \bm{Q})^{\dagger}\bm{\Psi}^T\bm{A}$. Hence, following the argument of \cite{nakatsukasa2020fast} we get
\begin{align*}
    &\|\bm{A}-\widetilde{\bm{A}}\|_F^2 = \|\bm{Q}_{\bot}\bm{Q}_{\bot}^T \bm{A} + (\bm{Q}\bm{Q}^T\bm{A}-\widetilde{\bm{A}})\|_F^2\\
    = & \|\bm{Q}_{\bot}\bm{Q}_{\bot}^T \bm{A}\|_F^2 + \|\bm{Q}\bm{Q}^T\bm{A}-\widetilde{\bm{A}}\|_F^2 + 2\tr(\bm{A}^T\bm{Q}_{\bot}\bm{Q}_{\bot}^T\widetilde{\bm{A}})\\
    = & \|\bm{Q}_{\bot}\bm{Q}_{\bot}^T \bm{A}\|_F^2 + \|\bm{Q}\bm{Q}^T\bm{A}-\widetilde{\bm{A}}\|_F^2,
\end{align*}
where the final inequality holds because $2\tr(\bm{A}^T\bm{Q}_{\bot}\bm{Q}_{\bot}^T\widetilde{\bm{A}}) = 0$, a consequence of $\bm{Q}^T_{\bot}\bm{Q} = 0$. The first term $\|\bm{Q}_{\bot}\bm{Q}_{\bot}^T \bm{A}\|_F^2$ is the error from the randomized SVD, which we can bound. Hence we only need to bound the second term. We have,
\begin{align*}
    &\|\bm{Q}\bm{Q}^T\bm{A}-\widetilde{\bm{A}}\|_F^2 = \|\bm{Q}(\bm{Q}^T - (\bm{\Psi}^T \bm{Q})^{\dagger}\bm{\Psi}^T)\bm{A}\|_F^2 = \|\bm{Q}((\bm{\Psi}^T \bm{Q})^{\dagger} (\bm{\Psi}^T \bm{Q}_{\bot}))\bm{Q}_{\bot}^T\bm{A}\|_F^2\\
    = & \|(\bm{\Psi}^T \bm{Q})^{\dagger} (\bm{\Psi}^T \bm{Q}_{\bot})\bm{Q}_{\bot}^T\bm{A}\|_F^2.
\end{align*}
Now let 
\begin{equation*}
    \bm{Y}_1 = \bm{Q}^T\bm{\Psi}, \quad \bm{Y}_2 = \bm{Q}^T_{\bot}\bm{\Psi}.
\end{equation*}
Once we condition on $\bm{\Omega}$, we know
\begin{equation*}
    \begin{bmatrix} \bm{Y}_1\\\bm{Y}_2 \end{bmatrix} \sim N(\bm{0},\widetilde{\bm{S}}),
\end{equation*}
where
\begin{equation*}
    \widetilde{\bm{S}} = \begin{bmatrix} \bm{Q}^T \bm{S} \bm{Q} & \bm{Q}^T \bm{S} \bm{Q}_{\bot}\\\bm{Q}_{\bot}^T \bm{S} \bm{Q} & \bm{Q}_{\bot}^T \bm{S} \bm{Q}_{\bot} \end{bmatrix} = \begin{bmatrix} \widetilde{\bm{S}}_{11} & \widetilde{\bm{S}}_{21}^T\\\widetilde{\bm{S}}_{21} & \widetilde{\bm{S}}_{22} \end{bmatrix}.
\end{equation*}
Note that $\widetilde{\bm{S}}$ is random and depends on $\bm{\Omega}$. We have
\begin{equation*}
    \|(\bm{\Psi}^T \bm{Q})^{\dagger} (\bm{\Psi}^T \bm{Q}_{\bot})\bm{Q}_{\bot}^T\bm{A}\|_F^2 = \|(\bm{A}^T \bm{Q}_{\bot})\bm{Y}_2 \bm{Y}_1^{\dagger}\|_F^2
\end{equation*}
Using the exact same argument as when we compute $\|\bm{\Sigma}_2\bm{\Omega}_2\bm{\Omega}_1^{\dagger}\|_F^2$ in Theorem~\ref{theorem:frobenius_expectation_bound1} we get
\begin{align*}
    &\mathbb{E}\|(\bm{A}^T \bm{Q}_{\bot})\bm{Y}_2 \bm{Y}_1^{\dagger}|_F^2 = \mathbb{E}[\mathbb{E}[\|(\bm{A}^T \bm{Q}_{\bot})\bm{Y}_2 \bm{Y}_1^{\dagger}\|_F^2|\bm{\Omega}]]\\
    & = \mathbb{E}\left[\|\bm{A}^T \bm{Q}_{\bot} \widetilde{\bm{S}}_{21}\widetilde{\bm{S}}_{11}^{-1}\|_F^2 - \|\bm{A}^T \bm{Q}_{\bot} \widetilde{\bm{S}}_{21}\widetilde{\bm{S}}_{11}^{-1/2}\|_F^2 \frac{\tr(\widetilde{\bm{S}}_{11}^{-1})}{\ell - 1} + \tr(\bm{A}^T \bm{Q}_{\bot} \widetilde{\bm{S}}_{22} \bm{Q}_{\bot}^T \bm{A})\frac{\tr(\widetilde{\bm{S}}_{11}^{-1})}{\ell - 1}\right].
\end{align*}
Note that from the expression above we get back the results from \cite{nakatsukasa2020fast} if we choose $\bm{S} = \bm{I}$, since in this case $\widetilde{\bm{S}} = \bm{I}$ a.s. Using the same arguments as in Corollary~\ref{corollary:expectation_bound_rsvd} we can get
\begin{align*}
    &\mathbb{E}\left[\|\bm{A}^T \bm{Q}_{\bot} \widetilde{\bm{S}}_{21}\widetilde{\bm{S}}_{11}^{-1}\|_F^2 - \|\bm{A}^T \bm{Q}_{\bot} \widetilde{\bm{S}}_{21}\widetilde{\bm{S}}_{11}^{-1/2}\|_F^2 \frac{\tr(\widetilde{\bm{S}}_{11}^{-1})}{\ell - 1} + \tr(\bm{A}^T \bm{Q}_{\bot} \widetilde{\bm{S}}_{22} \bm{Q}_{\bot}^T \bm{A})\frac{\tr(\widetilde{\bm{S}}_{11}^{-1})}{\ell - 1}\right]\\
    \leq & \mathbb{E}\left[\tr(\widetilde{\bm{S}}_{11}^{-1}) \tr(\bm{A}^T\bm{Q}_{\bot} \widetilde{\bm{S}}_{22}\bm{Q}_{\bot}^T \bm{A})\right].
\end{align*}
We can bound 
\begin{equation*}
    \tr(\bm{A}^T\bm{Q}_{\bot} \widetilde{\bm{S}}_{22}\bm{Q}_{\bot}^T \bm{A}) \leq \|\widetilde{\bm{S}}_{22}\|_2 \|\bm{Q}_{\bot}^T \bm{A}\|_F^2. %\leq \|\bm{S}\|_2 \|\bm{Q}_{\bot}^T \bm{A}\|_F^2.
\end{equation*}
Hence, combining everything we get
\begin{equation*}
    \mathbb{E}\|\bm{A}-\widetilde{\bm{A}}\|_F^2 \leq \mathbb{E}\left[(1 + \|\widetilde{\bm{S}}_{22}\|_2 \tr(\widetilde{\bm{S}}_{11}^{-1})) \|\bm{Q}_{\bot}^T \bm{A}\|_F^2\right]
\end{equation*}
We can further bound $\|\widetilde{\bm{S}}_{22}\|_2 \leq \|\bm{S}\|_2$, but how do we bound $\tr(\widetilde{\bm{S}}_{11}^{-1})$ without getting a dependence on the smallest eigenvalues of $\bm{S}$? 
%\subsection{Structural bound}
%By following the proof of \cite[Theorem 3.2]{nakatsukasa2020fast} we see that 
%\begin{lemma}
%\begin{equation*}
%    \|\bm{A}-\widetilde{\bm{A}}\|_F^2 = \|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_F^2 + \|(\bm{\Psi}^T\bm{Q})^{\dagger}((\bm{\Psi}^T\bm{Q}_{\bot})^{\dagger})\bm{Q}_{\bot}^T\bm{A}\|_F^2 + 2\tr(\bm{Q}(\bm{\Psi}^T\bm{Q})^{\dagger}((\bm{\Psi}^T\bm{Q}_{\bot})\bm{Q}_{\bot}^T\bm{A})
%\end{equation*}
%where $\bm{Q} = \texttt{orth}(\bm{A\Omega})$ and $\bm{Q}_{\bot}$ is an orthonormal basis spanning the orthogonal complement of $\range(\bm{Q})$. Note that $\bm{\Psi}$ is independent of $\bm{Q}$ and once we condition on $\bm{\Omega}$ $\bm{\Psi}^T\bm{Q}$ and $\bm{\Psi}^T\bm{Q}_{\bot}$ are Gaussians. 
%\end{lemma}

==> Notes/finitedim_nystrom.tex <==
\section{The finite dimensional symmetric Nyström approximation}

\subsection{Structural bound}
Let $\bm{A}$ be SPSD and define
\begin{equation*}
    \widehat{\bm{A}} = \bm{A}\bm{\Omega}(\bm{\Omega}^T \bm{A} \bm{\Omega})^{\dagger}(\bm{A}\bm{\Omega})^T
\end{equation*}
to be the Nyström approximation of $\bm{A}$. Hence,
\begin{equation*}
    \bm{A} - \widehat{\bm{A}} = \bm{A}^{1/2}(\bm{I}-\bm{P}_{\bm{A}^{1/2} \bm{\Omega}}) \bm{A}^{1/2},
\end{equation*}
where $\bm{P}_{\bm{B}}$ denotes the orthogonal projector onto $\range(\bm{B})$.
\begin{lemma}\label{lemma:structural_bound_nystrom}
Let $\|\cdot\|$ be any unitarily invariant norm. Then, if $\bm{\Omega}_1$ has full row-rank we have
\begin{equation*}
    \|\bm{A} - \widehat{\bm{A}}\| \leq \|\bm{\Sigma}_2\| + \|(\bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger})^T \bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger}\|.
\end{equation*}
\end{lemma}
\begin{proof}
This follows from applying \cite[Lemma 3.13]{persson2022randomized} with $q = 1$ to the operator monotone function $f(x) = x$. 
%As always, we can assume that $\bm{A} = \bm{\Sigma}$. Let
%\begin{equation*}
 %   \bm{Z} = \bm{\Sigma}_2^{1/2} \bm{\Omega} \bm{\Omega}_1^{\dagger}\bm{\Sigma}_1^{-1/2} = \begin{bmatrix} \bm{I}\\ \bm{\Sigma}_2^{1/2} \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\bm{\Sigma}_1^{-1/2} \end{bmatrix} = \begin{bmatrix} \bm{I}\\ \bm{F} \end{bmatrix}.
%\end{equation*}
%Then, $\range(\bm{\Sigma}^{1/2}\bm{\Omega}) \supseteq \range(\bm{Z})$ so $\bm{A}^{1/2}(\bm{I}-\bm{P}_{\bm{A}^{1/2} \bm{\Omega}}) \bm{A}^{1/2} \succeq \bm{A}^{1/2}(\bm{I}-\bm{P}_{\bm{Z}}) \bm{A}^{1/2}$ and
%\begin{equation*}
%    \|\bm{A} - \widehat{\bm{A}}\|_F \leq \|\bm{A}^{1/2}(\bm{I}-\bm{P}_{\bm{Z}}) \bm{A}^{1/2}\|.
%\end{equation*}
%We know that 
%\begin{equation*}
%    \bm{I}-\bm{P}_{\bm{Z}} = \begin{bmatrix} \bm{I}-(\bm{I}-\bm{F}^T \bm{F})^{-1} & * \\ * & \bm{I}-\bm{F}(\bm{I}-\bm{F}^T \bm{F})^{-1}\bm{F}^T \end{bmatrix}.
%\end{equation*}
%Hence,
%\begin{equation*}
 %   \bm{A}^{1/2}(\bm{I}-\bm{P}_{\bm{Z}}) \bm{A}^{1/2} = \begin{bmatrix} \bm{\Sigma}_1^{1/2}(\bm{I}-(\bm{I}-\bm{F}^T \bm{F})^{-1})\bm{\Sigma}_1^{1/2} & * \\ * & \bm{\Sigma}_2^{1/2}(\bm{I}-\bm{F}(\bm{I}-\bm{F}^T \bm{F})^{-1}\bm{F}^T)\bm{\Sigma}_2^{1/2} \end{bmatrix}.
%\end{equation*}
%Note by Lemma~\ref{lemma:partition_spsd} we have
%\begin{align*}
 %   & \|\bm{A}^{1/2}(\bm{I}-\bm{P}_{\bm{Z}}) \bm{A}^{1/2}\| \leq \|\bm{\Sigma}_1^{1/2}(\bm{I}-(\bm{I}-\bm{F}^T \bm{F})^{-1})\bm{\Sigma}_1^{1/2}\| + \|\bm{\Sigma}_2^{1/2}(\bm{I}-\bm{F}(\bm{I}-\bm{F}^T \bm{F})^{-1}\bm{F}^T)\bm{\Sigma}_2^{1/2}\|\\
  %  \leq & \|\bm{\Sigma}_2\| + \|\bm{\Sigma}_1^{1/2}\bm{F}^T \bm{F} \bm{\Sigma}_1^{1/2}\| = \|\bm{\Sigma}_2\| + \|(\bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger})^T \bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger}\|
%\end{align*}
\end{proof}
\begin{remark}
We can obtain the following structural bound for the spectral norm, Frobenius norm and nuclear norm respectively
\begin{align*}
     &\|\bm{A} - \widehat{\bm{A}}\|_2 \leq + \|\bm{\Sigma}_2\|_2 + \|(\bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger})^T \bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger}\|_2 = \|\bm{\Sigma}_2\|_2 + \|\bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger}\|_2^2;\\
     &  \|\bm{A} - \widehat{\bm{A}}\|_F \leq + \|\bm{\Sigma}_2\|_F + \|(\bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger})^T \bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger}\|_F = \|\bm{\Sigma}_2\|_F + \|\bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^2;\\
     &\|\bm{A} - \widehat{\bm{A}}\|_* \leq + \|\bm{\Sigma}_2\|_* + \|(\bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger})^T \bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger}\|_* = \|\bm{\Sigma}_2\|_* + \|\bm{\Sigma}_2^{1/2}\bm{\bm{\Omega}}_2 \bm{\Omega}_1^{\dagger}\|_F^2
\end{align*}
\end{remark}

%\begin{remark}
%Perhaps an easier way of deriving the structural bound is by noting that $\|\bm{A}-\widehat{\bm{A}}\|_{(p)} = \|(\bm{I}-\bm{P}_{\bm{A}^{1/2}\bm{\Omega}})\bm{A}^{1/2}\|_{(2p)}^2$, and then use results for the structural bounds in arbitrary Schatten norms. See \cite{saibaba_subspace}. 
%\end{remark}

\subsection{Expectation bounds}
Prepatory lemmas.
\begin{lemma}\label{lemma:shifted_4norm}
Consider $\bm{C} \in \mathbb{R}^{m_1 \times m_2}, \bm{D} \in \mathbb{R}^{n_1 \times n_2}$ and a standard Gaussian $m_2 \times n_1$ matrix $\bm{\Psi}$. Define $\bm{\Phi} = \bm{C}\bm{\bm{\Psi}}\bm{D}$. Given any matrix $\bm{B} \in \mathbb{R}^{m_1 \times n_2}$ we have
\begin{align*}
    &\mathbb{E}\|\bm{B}+\bm{\Phi}\|_{(4)}^4 = \|\bm{B}\|_{(4)}^4 + \|\bm{C}\|_{(4)}^4\|\bm{D}\|_{(4)}^4 + \|\bm{C}\|_{F}^4\|\bm{D}\|_{(4)}^4 + \|\bm{C}\|_{(4)}^4\|\bm{D}\|_{F}^4 +\\ &2\left(\|\bm{B}^T \bm{C}\|_F^2 \|\bm{D}\|_F^2 + \|\bm{C}\|_F^2 \|\bm{D}\bm{B}^T\|_F^2 + \|\bm{C}^T \bm{B}\bm{D}^T\|_F^2\right).
\end{align*}
\end{lemma}
\begin{lemma}\label{lemma:inversewishart_norm_expectation}
If $p \geq 4$ we have
\begin{equation*}
    \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_F^4 = \frac{(p-2)\tr(\widetilde{\bm{K}}_{11}^{-1})^2 + 2 \|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{p(p-1)(p-3)},
\end{equation*}
and
\begin{equation*}
    \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_{(4)}^4 = \frac{\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{p(p-3)} + \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})^2}{p(p-1)(p-3)}.
\end{equation*}
\end{lemma}
\quad\\
Lemmas above are proved in Appendix~\ref{section:lemma_shifted_4norm} and Appendix~\ref{section:proof_inversewishart_norm_expectation}.\\\\
Prepatory lemma.
\begin{lemma}\label{lemma:inverse_product}
Let $\bm{B}$ be an arbitrary matrix. Then, if $p \geq 2$
\begin{equation*}
    \mathbb{E}\|\bm{\Omega}_1^{\dagger}\bm{B}\|_F^2 = \frac{\tr(\bm{B}^T \widetilde{\bm{K}}_{11}^{-1} \bm{B})}{p-1} = \frac{\|\bm{B}^T \widetilde{\bm{K}}_{11}^{-1/2}\|_F^2}{p-1}.
\end{equation*}
\end{lemma}
\begin{proof}
Let $\bm{X} = \bm{\Omega}_1\bm{\Omega}_1^T \sim \mathcal{W}_{k}(\widetilde{\bm{K}}_{11},k+p)$. Then,
\begin{equation*}
    \|\bm{\Omega}_1^{\dagger}\bm{B}\|_F^2 = \tr(\bm{B}^T \bm{X}^{-1}\bm{B}).
\end{equation*}
The result is obtained by applying Lemma\ref{lemma:gaussian_facts}~(\ref{lemma:inversewishart_expectation}).
\end{proof}

\begin{lemma}\label{lemma:loewner}
Let $\bm{B}, \bm{C}$ and $\bm{D}$ be positive semi-definite matrices. Assume $\bm{B} \succeq \bm{C}$. Then,
\begin{equation*}
    \langle \bm{C}, \bm{D} \rangle \leq \langle \bm{B}, \bm{D} \rangle.
\end{equation*}
\end{lemma}
\begin{proof}
    Since $\bm{D} \succeq \bm{0}$ it has a uniquely defined square-root. Furthermore, by \cite[Theorem 7.7.2 (a) and Corollary 7.7.4 (d)]{matrixanalysis} we have
    \begin{align*}
        \langle \bm{C}, \bm{D} \rangle = \tr(\bm{C}\bm{D}) = \tr(\bm{D}^{1/2}\bm{C}\bm{D}^{1/2}) \leq \tr(\bm{D}^{1/2}\bm{B}\bm{D}^{1/2}) =  \langle \bm{B}, \bm{D} \rangle,
    \end{align*}
    as required. 
\end{proof}

\quad\\
Main result.

\begin{theorem}\label{theorem:expectation_nystrom}
Let us denote
\begin{align*}
    \alpha_1 &= \frac{(p-1)k^2 + (p+1)k}{p(p-1)(p-3)} = O\left(\frac{k^2}{p^2}\right);\\
    \alpha_2 &= \frac{k(p-1) + k^2}{p(p-1)(p-3)} = O\left(\frac{kp + k^2}{p^3}\right);\\
    \alpha_3 &= \frac{2k}{p-1} = O\left(\frac{k}{p}\right);\\
    \alpha_4 &= \frac{2}{p-1} = O\left(\frac{1}{p}\right).
\end{align*}
Define
\begin{equation*}
    \beta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \delta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \xi \in \{F,*\},
\end{equation*}
and
\begin{equation*}
    \gamma_k = \frac{1}{\lambda_1 \|\bm{\widetilde{\bm{K}}}_{11}^{-1}\|_2}.
\end{equation*}
Then, if $p \geq 4$
\begin{equation*}
    \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \left((1 + \sqrt{\alpha_1} \frac{\beta_k^{(F)}}{\gamma_k} + \left(1+\frac{\alpha_3 + \alpha_4}{\sqrt{\alpha_1}}\right)\frac{\delta_k^{(F)}}{\gamma_k}\right) \|\bm{\Sigma}_2\|_F + \left(\sqrt{\alpha_2} \frac{\beta_k^{(*)}}{\gamma_k} + \frac{\alpha_4}{\sqrt{\alpha_2}} \frac{\delta_k^{(*)}}{\gamma_k}\right)\|\bm{\Sigma}_2\|_*,
\end{equation*}
%\begin{align*}
 %   & \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F \\
    %+& \left(\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 + (C_1+C_2)\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4 + C_1\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4 +\right.\\
    %&\left. 2 \|\widetilde{\bm{K}}_{22.1}^{1/2}\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} + 2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \frac{\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2}{p-1} + 2\frac{\|\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Sigma}_2 \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2}{p-1}\right)^{1/2}
%\end{align*}
\end{theorem}

\begin{proof}
From Lemma~\ref{lemma:structural_bound_nystrom} and Hölder's inequality we only need to bound $\sqrt{\mathbb{E}\|\bm{\Sigma}_1^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^4}$. Let $\bm{\Psi}$ denote a standard Gaussian matrix. Then, 
\begin{align*}
    &\mathbb{E}\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^4 = \mathbb{E}\left[\mathbb{E}\left[\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^4|\bm{\Omega}_1\right]\right] \\
    = & \mathbb{E}\left[\mathbb{E}\left[\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} + \bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Psi}\bm{\Omega}_1^{\dagger}\|_{(4)}^4|\bm{\Omega}_1\right]\right] && \text{(Lemma~\ref{lemma:gaussian_facts}~(\ref{lemma:cond_distribution}))}\\
    = & \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 + \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4 \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_{(4)}^4 \\
    + &\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4 \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_{(4)}^4 + \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4 \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_{F}^4\\
    + & 2\|\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Sigma}_2 \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_F^2 \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_F^2 + 2 \|\bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2 \mathbb{E}\|\bm{\Omega}_1^{\dagger}\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2}\|_F^2 \\
    + &2 \mathbb{E}\|\bm{\Omega}_1^{\dagger}\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2. && (\text{Lemma~\ref{lemma:shifted_4norm}}) 
\end{align*}
The terms in the expectations are known from Lemma~\ref{lemma:frobeniusinverse_expectation}, Lemma~\ref{lemma:inversewishart_norm_expectation} and Lemma~\ref{lemma:inverse_product}, which yields the following bound.

\begin{align}\label{eq:nystrom_expectationbound1}
\begin{split}
    & \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F + \left(\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 \right.\\
    + & \left. (\beta_1 + \beta_2)\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4 +  \beta_1\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4 \right.\\
    + & \left. \alpha_4 \|\widetilde{\bm{K}}_{22.1}^{1/2}\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 \tr(\widetilde{\bm{K}}_{11}^{-1}) \right.\\
    + & \left. \alpha_4\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2 + \alpha_4\|\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Sigma}_2 \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2\right)^{1/2}
\end{split}
\end{align}
where
\begin{equation*}
    \beta_1 = \frac{\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{p(p-3)} + \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})^2}{p(p-1)(p-3)}, \quad \beta_2 = \frac{(p-2)\tr(\widetilde{\bm{K}}_{11}^{-1})^2 + 2\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{p(p-1)(p-3)}.
\end{equation*}
We will now bound each of the six terms inside the square-root on the right hand side of \eqref{eq:nystrom_expectationbound1}. Using strong submultiplicativity of Schatten norms, $\|\bm{B}\|_{(2p)}^{2p} = \|\bm{B}\bm{B}^T\|_{(p)}^{p}$ for $p \in [1, \infty)$, $\|\bm{B}\bm{B}^T\|_2 = \|\bm{B}\|_2^2$, and norm equivalences we obtain
\begin{align}
    &\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 \leq \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}\|_{F}^2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2; \label{eq:1}\\
    & (\beta_1+\beta_2)\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4 = \alpha_1\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2}\|_{F}^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2;\label{eq:2}\\
    & \beta_1\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4 = \alpha_2\tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2})^2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2;\label{eq:3}\\
    \begin{split}&\alpha_4\|\widetilde{\bm{K}}_{22.1}^{1/2}\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2\tr(\widetilde{\bm{K}}_{11}^{-1}) \\
     &\leq  \alpha_3\langle  \bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1} \bm{\Sigma}_2^{1/2}, \bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2}\rangle\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2;\label{eq:4}\end{split}\\\begin{split}
    & \alpha_4 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2 \\
    & \leq \alpha_4 \tr(\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1} \bm{\Sigma}_2^{1/2}) \tr(\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}) \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2;\label{eq:5}\end{split}\\
    \begin{split}& \alpha_4\|\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Sigma}_2 \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2 \\
     &\leq \alpha_4\langle  \bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1} \bm{\Sigma}_2^{1/2}, \bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2}\rangle\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2. \label{eq:6}\end{split}
\end{align}
Since $\widetilde{\bm{K}_{21}} \widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}_{21}}^T \succeq 0$ we have
\begin{align*}
    \eqref{eq:3} + \eqref{eq:5} = \alpha_2&\left(\tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}) - \tr(\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}) \right)\\
    \cdot &\left(\tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}) + (\frac{\alpha_4}{\alpha_2}-1) \tr(\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}) \right) \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2\\
    \leq & \alpha_2\left(\tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}) + \frac{\alpha_4}{\alpha_2} \tr(\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}) \right)^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2.
\end{align*}
Since $\widetilde{\bm{K}}_{22} \succeq \widetilde{\bm{K}}_{22.1} \succeq \bm{0}$ we have by \cite[Lemma 3.1 (i)]{persson2022randomized} and Lemma~\ref{lemma:loewner}
\begin{align}
    \eqref{eq:2} &\leq \alpha_1 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2;\label{eq:2inequality}\\
    \eqref{eq:4} + \eqref{eq:6} &\leq \langle  \bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22} \bm{\Sigma}_2^{1/2}, (\alpha_3  + \alpha_4)\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2}\rangle\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2\label{eq:4+6inequality}.
\end{align}
Consequently,
\begin{align*}
    &\eqref{eq:2} + \eqref{eq:4} + \eqref{eq:6} \\
    \leq & \langle  \bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22} \bm{\Sigma}_2^{1/2}, (\alpha_3  + \alpha_4)\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2} + \alpha_1 \bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\rangle\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2\\
    \leq & \|  \bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22} \bm{\Sigma}_2^{1/2}\|_F \|(\alpha_3  + \alpha_4)\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2} + \alpha_1 \bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2\\
    \leq & \alpha_1 \|\frac{\alpha_3  + \alpha_4}{\alpha_1}\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2} + \bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2\\
    \leq & \alpha_1\left(\frac{\alpha_3  + \alpha_4}{\alpha_1}\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2}\|_F + \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F\right)^2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2,
\end{align*}
where the first inequality is due to \eqref{eq:2inequality}
 and \eqref{eq:4+6inequality}, the second inequality is due to the Cauchy-Schwartz inequality, the third inequality is due to \cite[Lemma 3.1 (i)]{persson2022randomized}, and the fourth inequality is due to the triangle inuquality. Combining the derived inequalities for $\eqref{eq:1} + \ldots + \eqref{eq:6}$ and using the subadditivity of the square-root we obtain
\begin{align*}
    & \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F \\
    +& \left(\sqrt{\alpha_1} \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F + \left(1+\frac{\alpha_3 + \alpha_4}{\sqrt{\alpha_1}}\right)\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2}\|_F\right.\\
      + & \left.\sqrt{\alpha_2}\tr(\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22} \bm{\Sigma}_2^{1/2}) + \frac{\alpha_4}{\sqrt{\alpha_2}} \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2})\right)  \|\widetilde{\bm{K}}_{11}^{-1}\|_2\\
      = & \left(1 + \sqrt{\alpha_1} \frac{\beta_k^{(F)}}{\gamma_k} + \left(1+\frac{\alpha_3 + \alpha_4}{\sqrt{\alpha_1}}\right)\frac{\delta_k^{(F)}}{\gamma_k}\right) \|\bm{\Sigma}_2\|_F + \left(\sqrt{\alpha_2} \frac{\beta_k^{(*)}}{\gamma_k} + \frac{\alpha_4}{\sqrt{\alpha_2}} \frac{\delta_k^{(*)}}{\gamma_k}\right)\|\bm{\Sigma}_2\|_*,
\end{align*}
as required.

\end{proof}

\begin{remark}
In the ideal scenario $\widetilde{\bm{K}}$ is block-diagonal with $\widetilde{\bm{K}}_{11}$ as the only non-zero block. In this case Theorem~\ref{theorem:expectation_nystrom} tells us that $\mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F$. I.e., if we choose $\bm{K}$ optimally, we obtain the best low-rank approximation. 
\end{remark}

\begin{corollary}
In the setting of Theorem~\ref{theorem:frobenius_expectation_bound1} with $\bm{K} = \bm{I}$ we obtain
\begin{equation*}
    \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \left(1 + \frac{(p-1)k^2 + (p+1)k}{p(p-1)(p-3)}\right)^{1/2}\|\bm{\Sigma}_2\|_F + \left(\frac{k^2 + (p-1)k}{p(p-1)(p-3)}\right)^{1/2}\|\bm{\Sigma}_2\|_*.
\end{equation*} 
\end{corollary}
%\begin{proof}
%This holds because when $\bm{K} = \bm{I}$ we have
%\begin{equation*}
 %   C_1 = \frac{k^2 + k(p-1)}{p(p-1)(p-3)}, \quad C_2 = \frac{(p-2)k^2 + 2k}{p(p-1)(p-3)},
%\end{equation*}
%any terms involving $\widetilde{\bm{K}}_{21}$ disappear and $\widetilde{\bm{K}}_{22.1} = \bm{I}$. 
%\end{proof}

\begin{remark}
Note that if we choose $p = O(k)$ and $\bm{K} = \bm{I}$ we have
\begin{equation*}
    \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq (1 + O(1))\|\bm{\Sigma}_2\|_F + O\left(\frac{1}{\sqrt{k}}\right) \|\bm{\Sigma}_2\|_*.
\end{equation*}
\end{remark}
%Main result: nicer version.
%\begin{theorem}\label{theorem:expectation_nystrom2}
%Define 
%\begin{align*}
 %   q_0(p) &= 1+\frac{2}{p-1} = O(1);\\
  %  q_1(p) &= \frac{2}{p-1} = O(p^{-1});\\
   % q_2(p) &= \frac{1}{p(p-3)} = O(p^{-2});\\
    %q_3(p) & = \frac{1}{p(p-1)(p-3)} = O(p^{-3});\\
    %\alpha^2 &= q_0(p) \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2 + 2q_2(p) \|\widetilde{\bm{K}}_{11}^{-1}\|_F^2 + q_1(p) \|\widetilde{\bm{K}}_{11}^{-1}\|_2\tr(\widetilde{\bm{K}}_{11}^{-1}) + q_2(p) \tr(\widetilde{\bm{K}}_{11}^{-1})^2;\\
    %\beta^2 &= q_1(p) \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2 + q_2(p) \|\widetilde{\bm{K}}_{11}^{-1}\|_F^2 + q_3(p) \tr(\widetilde{\bm{K}}_{11}^{-1})^2.
%\end{align*}
%Then, if $p \geq 4$
%\begin{equation*}
 %   \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F + \alpha \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F + \beta \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}).
%\end{equation*}
%\end{theorem}

%\begin{proof}
%Using the fact that $\widetilde{\bm{K}}_{22} \succeq \widetilde{\bm{K}}_{22.1}, \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T$ and strong submultiplicativity of Schatten norms we have from Lemma~\ref{theorem:expectation_nystrom}\footnote{Reminder to David: For the third inequality, write out the Frobenius norm explicitly, and use that the Schur complement is psd.}
%\begin{align*}
    %\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 &\leq \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2\\
    %(C_1 + C_2)\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4 &\leq (C_1 + C_2)\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2\\
    %C_1\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4 &\leq C_1 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})^2\\
    %2 \|\widetilde{\bm{K}}_{22.1}^{1/2}\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} & \leq  \frac{2\|\widetilde{\bm{K}}_{11}^{-1}\|_2\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2\\
    %2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \frac{\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2}{p-1} & \leq \frac{2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2}{p-1}\tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})^2\\ \frac{2\|\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Sigma}_2 \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2}{p-1}  &\leq  \frac{2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2}{p-1}\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2.
%\end{align*}
%Summing over we get\footnote{For the term involving $\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2$ we need to bound $\frac{p+1}{p(p-1)(p-3)} \leq 2 q_2(p)$.} \begin{align*}
    %&\mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F\\
   %+ & \left(\alpha^2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2 + \beta^2\tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})^2 \right)^{1/2}.
%\end{align*}
%Subadditivity of the square-root yields the result.
%\end{proof}

%Main result: nice version.
%\begin{corollary}
%Let $p = k \geq 4$, and define
%Then,
%\begin{equation*}
 %   \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F + \left(O(1) \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F + O\left(\frac{1}{\sqrt{k}}\right)\tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})\right)\|\widetilde{\bm{K}}_{11}^{-1}\|_2.
%\end{equation*}
%Furthermore, if we define
%\begin{equation*}
 %   \beta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \xi \in \{F,*\},
%\end{equation*}
%and
%\begin{equation*}
 %   \gamma_k = \frac{1}{\lambda_1 \|\bm{\widetilde{\bm{K}}}_{11}^{-1}\|_2}.
%\end{equation*}
%Then, 
%\begin{equation*}
 %   \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \left(1 + \sqrt{1 + \frac{3k^2 -3k -8}{(k-1)(k-3)}} \frac{\beta_k^{(F)}}{\gamma_k}\right)\|\bm{\Sigma}_2\|_F + \sqrt{\frac{4k-7}{(k-1)(k-3)}} \frac{\beta_k^{(*)}}{\gamma_k}\|\bm{\Sigma}_2\|_*.
%\end{equation*}
%where the hidden quantities are $\sqrt{1 + \frac{3k^2 -3k -8}{(k-1)(k-3)}} = O(1)$ and $\sqrt{\frac{4k-7}{(k-1)(k-3)}} = O(k^{-1/2})$.
%\end{corollary}
%\begin{proof}
%Using the fact that $\widetilde{\bm{K}}_{22} \succeq \widetilde{\bm{K}}_{22.1}, \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T$ and strong submultiplicativity of Schatten norms we have from Lemma~\ref{theorem:expectation_nystrom}%\footnote{Reminder to David: For the third inequality, write out the Frobenius norm explicitly, and use that the Schur complement is psd.}
%\begin{align*}
    %\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 &\leq \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2\\
    %(C_1 + C_2)\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4 &\leq (C_1 + C_2)\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2\\
    %C_1\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4 &\leq C_1 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})^2\\
    %2 \|\widetilde{\bm{K}}_{22.1}^{1/2}\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} & \leq  \frac{2\|\widetilde{\bm{K}}_{11}^{-1}\|_2\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2\\
    %2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \frac{\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2}{p-1} & \leq \frac{2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2}{p-1}\tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})^2\\ \frac{2\|\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Sigma}_2 \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2}{p-1}  &\leq  \frac{2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2}{p-1}\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2.
%\end{align*}
%Using the fact that $k = p$ %we can bound 
%\begin{align*}
    %\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2 &\leq k\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2;\\
    %\|\widetilde{\bm{K}}_{11}^{-1}\|_2\tr(\widetilde{\bm{K}}_{11}^{-1}) & \leq k\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2;\\
    %\tr(\widetilde{\bm{K}}_{11}^{-1})^2 \leq & k^2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2.
%\end{align*}
%Inserting the derived inequalities into the bound in Theorem~\ref{theorem:expectation_nystrom} and the subadditivity of the square-root yields the result. 
%\end{proof}

%\begin{remark}
%Arguably, Theorem~\ref{theorem:expectation_nystrom} and Theorem~\ref{theorem:expectation_nystrom2} are complicated. An easier way of obtaining an expectation bound is by bounding
%\begin{align*}
    %&\mathbb{E}\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2\bm{\Omega}_1^{\dagger}\|_{(4)}^2 \leq \sqrt{\mathbb{E}|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2\|_{(4)}^4}\sqrt{\mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_{(4)}^4}\\
    %= & \sqrt{\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}^{1/2}\|_{(4)}^4(k+p) + \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}^{1/2}\|_{F}^4(k+p) + \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}^{1/2}\|_{(4)}^4(k+p)^2} \\
    %\times& \sqrt{\frac{\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{p(p-3)} + \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})^2}{p(p-1)(p-3)}}\\
    %= & \sqrt{\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_{F}^2(k+p) + \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})^2(k+p) + \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_{F}^2(k+p)^2} \\
    %\times& \sqrt{\frac{\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{p(p-3)} + \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})^2}{p(p-1)(p-3)}}.
%\end{align*}
%Thus by letting $\alpha = \sqrt{\frac{\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{p(p-3)}+ \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})^2}{p(p-1)(p-3)}}$ we have, by using subadditivity of the square-root
%\begin{align*}
    %&\mathbb{E}\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2\bm{\Omega}_1^{\dagger}\|_{(4)}^2 \leq\\
    %& \alpha \left(\sqrt{(k+p)^2 + k+p} \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F + \sqrt{k+p}\tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})\right),
%\end{align*}
%but this would not recover the case when $\bm{K} = \bm{I}$ and is not necessarily more interpretable.
%\end{remark}

\subsection{Tailbounds}
Preliminary lemmas.
\begin{lemma}\label{lemma:omega1_tailbound}
Let $p \geq 4$. Then,
\begin{align*}
    &\mathbb{P}\left(\|\bm{\Omega}_1^{\dagger}\|_F > \sqrt{\frac{3\tr(\widetilde{\bm{K}}_{11}^{-1})}{p+1}} t\right) \leq t^{-p};\\
    & \mathbb{P}\left(\|\bm{\Omega}_1^{\dagger}\|_{(4)} > \frac{e \sqrt{(k+p) \|\widetilde{\bm{K}}_{11}^{-1}\|_F}}{p+1} t\right) \leq t^{-(p+1)};\\
    & \mathbb{P}\left(\|\bm{\Omega}_1^{\dagger}\|_{2} > \frac{e \sqrt{(k+p) \|\widetilde{\bm{K}}_{11}^{-1}\|_2}}{p+1} t\right) \leq t^{-(p+1)}.
\end{align*}

\end{lemma}
The first is from \cite[Lemma 3]{boulle2022learning}. The other two are proved in Appendix~\ref{appendix:proof_omega1_tailbounds}.\\
\quad\\
Main theorem.
\begin{theorem}\label{theorem:nystrom_tailbound1}
Let us denote
\begin{align*}
    \alpha_1 &= \frac{e^2(k+p)}{(p+1)^2};\\
    \alpha_2 & = \frac{k}{p+1};\\
    \alpha_3 & = 9 \alpha_2^2 + k \alpha_1^2;\\
    \alpha_4 & = k \alpha_1^2.
\end{align*}
Define
\begin{equation*}
    \beta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \delta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \xi \in \{2,F,*\},
\end{equation*}
and
\begin{equation*}
    \gamma_k = \frac{1}{\lambda_1 \|\bm{\widetilde{\bm{K}}}_{11}^{-1}\|_2}.
\end{equation*}
Assume that $p \geq 4$ and $u,t > 1$. Then with probability at least $1-3t^{-p}-e^{-u^2/2}$ we have
\begin{align*}
    \|\bm{A}-\widehat{\bm{A}}\|_F \leq &\|\bm{\Sigma}_2\|_F + 2 \alpha_1 t^2 u^2 \frac{\beta_k^{(2)}}{\gamma_k} \|\bm{\Sigma}_2\|_2 + 2\left( \sqrt{\alpha_3} t^2\frac{\beta_k^{(2)}}{\gamma_k} + \left(1 + \frac{6\alpha_2}{\sqrt{\alpha_3}}\right) \frac{\delta_k^{(2)}}{\gamma_k}\right)\|\bm{\Sigma}_2\|_F\\
    + & 2\left(\sqrt{\alpha_4} t^2 \frac{\beta_k^{(*)}}{\gamma_k} + \frac{4\alpha_1}{\sqrt{\alpha_4}} \frac{\delta_k^{(*)}}{\gamma_k}\right)\|\bm{\Sigma}_2\|_*
\end{align*}
%\begin{align*}
    %&\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F + \frac{2e^2(k+p)}{(p+1)^2}\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_2^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_2 t^2 u^2\\
    %+ & 2\left(\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 + \|\bm{\Sigma}^{1/2}_2\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4\left(\frac{9\tr(\widetilde{\bm{K}}_{11}^{-1})^2}{(p+1)^2} + \frac{e^4\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2(k+p)^2}{(p+1)^4} \right)t^4\right.\\
    %+ & \left. \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4\frac{e^4\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2(k+p)^2}{(p+1)^4}t^4+ 2 \|\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2 \frac{3\tr(\widetilde{\bm{K}}_{11}^{-1})}{p+1} t^2\right.\\
    %+ &\left. 4\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{F}^2 \frac{e^2(k+p)\|\widetilde{\bm{K}}_{11}^{-1}\|_2 }{(p+1)^2} t^2\right)^{1/2}
%\end{align*}
\end{theorem}
\begin{proof}
Let $U(\bm{\Omega}_1)$ be an upper bound for $\mathbb{E}[\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}|\bm{\Omega}_1]$. Then,
\begin{align*}
    &\mathbb{P}\left(\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^2 \geq 2 U(\bm{\Omega}_1)^2 + 2u^2\|\bm{\Sigma}_2^{1/2}\bm{K}_{22.1}^{1/2}\|_2^2 \|\bm{\Omega}_1^{\dagger}\|_2^2 | \bm{\Omega}_1\right)\\
    \leq & \mathbb{P}\left(\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)} \geq  U(\bm{\Omega}_1) + u\|\bm{\Sigma}_2^{1/2}\bm{K}_{22.1}^{1/2}\|_2 \|\bm{\Omega}_1^{\dagger}\|_2 | \bm{\Omega}_1\right)\\
    \leq & \mathbb{P}\left(\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)} \geq  \mathbb{E}[\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}|\bm{\Omega}_1] + u\|\bm{\Sigma}_2^{1/2}\bm{K}_{22.1}^{1/2}\|_2 \|\bm{\Omega}_1^{\dagger}\|_2 | \bm{\Omega}_1\right) \leq e^{-u^2/2},
\end{align*}
where the first inequality comes from $2a^2 + 2b^2 \geq (a+b)^2$ and the final inequality comes from Lemma~\ref{lemma:tailbound_shifted_pnorm} and the fact that 
\begin{equation*}
    \|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}|\bm{\Omega}_1 \sim \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} + \bm{\Sigma}_2^{1/2}\bm{K}_{22.1}^{1/2} \bm{\Psi} \bm{\Omega}_1^{\dagger}\|_{(4)} | \bm{\Omega}_1.
\end{equation*}
By Lemma~\ref{lemma:shifted_4norm} and Hölder's inequality we we can set 
\begin{align*}
    U(\bm{\Omega}_1)^4 &= \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 + \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4\left(\|\bm{\Omega}_1^{\dagger}\|_{(4)}^4 + \|\bm{\Omega}_1^{\dagger}\|_{F}^4\right) + \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4\|\bm{\Omega}_1^{\dagger}\|_{(4)}^4\\
    +&2\|\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2\|\bm{\Omega}_1^{\dagger}\|_F^2 + 4 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_F^2 \|\bm{\Omega}_1^{\dagger}\|_2^2.
\end{align*}
Consider the event
\begin{equation*}
    E_t := \left\{\|\bm{\Omega}_1^{\dagger}\|_F \leq \sqrt{\frac{3\tr(\widetilde{\bm{K}}_{11}^{-1})}{p+1}} t, \|\bm{\Omega}_1^{\dagger}\|_{(4)} \leq \frac{e \sqrt{(k+p) \|\widetilde{\bm{K}}_{11}^{-1}\|_F}}{p+1}t, \|\bm{\Omega}_1^{\dagger}\|_{2} \leq \frac{e \sqrt{(k+p) \|\widetilde{\bm{K}}_{11}^{-1}\|_2}}{p+1}t\right\},
\end{equation*}
and let 
\begin{align*}
    U_t^4 & =  \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 + \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4\left(\frac{e^4(k+p)^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{(p+1)^4} + \frac{9 \tr(\widetilde{\bm{K}}_{11}^{-1})^2}{(p+1)^2}\right)t^4 \\
    + & \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4\frac{e^4(k+p)^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{(p+1)^4}t^4 +2\|\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \frac{3\tr(\widetilde{\bm{K}}_{11}^{-1})}{p+1}t^2 \\
    + & 4 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_F^2 \frac{e^2(k+p)\|\widetilde{\bm{K}}_{11}^{-1}\|_2}{(p+1)^2}t^2.
\end{align*}
Then,
\begin{equation*}
    \mathbb{P}\left(\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^2 \geq 2 U_t^2 + 2u^2t^2 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_2^2 \frac{e^2(k+p)\|\widetilde{\bm{K}}_{11}^{-1}\|_2}{(p+1)^2}| E_t\right) \leq e^{-u^2/2}
\end{equation*}
Furthermore, we have that $\mathbb{P}(E_t^c) \leq t^{-p} + 2t^{-(p+1)} \leq 3t^{-p}$ from Lemma~\ref{lemma:omega1_tailbound}. So we have
\begin{equation*}
    \mathbb{P}\left(\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^2 \geq 2 U_t^2 + 2u^2t^2 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_2^2 \frac{e^2(k+p)\|\widetilde{\bm{K}}_{11}^{-1}\|_2}{(p+1)^2}\right) \leq e^{-u^2/2} + 3t^{-p}.
\end{equation*}
Now it suffices to show that
\begin{align*}
    U_t^2 \leq &\sqrt{\alpha_3} t^2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22} \bm{\Sigma}_2^{1/2}\|_F\|\widetilde{\bm{K}}_{11}^{-1}\|_2 + (1+\frac{6\alpha_2}{\sqrt{\alpha_3}}) \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}\|_F\|\widetilde{\bm{K}}_{11}^{-1}\|_2\\
    + & \sqrt{\alpha_4} t^2 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22} \bm{\Sigma}_2^{1/2})\|\widetilde{\bm{K}}_{11}^{-1}\|_2 + \frac{4\alpha_1}{\sqrt{\alpha_4}} \tr(\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2^{1/2})\|\widetilde{\bm{K}}_{11}^{-1}\|_2.
\end{align*}
First note using norm equivalences and the definitions of $\alpha_1,\alpha_2, \alpha_3,$ and $\alpha_4$ we obtain
\begin{align*}
    U_t^4 & =  \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 + \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4\left(\frac{e^4(k+p)^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{(p+1)^4} + \frac{9 \tr(\widetilde{\bm{K}}_{11}^{-1})^2}{(p+1)^2}\right)t^4 \\
    + & \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4\frac{e^4(k+p)^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_F^2}{(p+1)^4}t^4 +2\|\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \frac{3\tr(\widetilde{\bm{K}}_{11}^{-1})}{p+1}t^2 \\
    + & 4 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_F^2 \frac{e^2(k+p)\|\widetilde{\bm{K}}_{11}^{-1}\|_2}{(p+1)^2}t^2\\
    \leq & \left(\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2} \|_F^2 + \alpha_3 t^4 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2} \|_F^2\right.\\
    + & \left. \alpha_4 t^4 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2})^2 + 6\alpha_2 t^2 \langle \bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2},\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\rangle\right.\\
    + & \left. 4\alpha_1 t^2 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2}) \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2})\right)\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2. 
\end{align*}
We will now bound each term on the right hand side of the bound for $U_t$. First we bound
\begin{align}\label{eq:inequality_tailbound1}
\begin{split}
    &\alpha_4 t^4 \tr(\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1} \bm{\Sigma}_2^{1/2})^2 + 4\alpha_1 t^2 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2}) \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2})\\
    = & \alpha_4 t^4 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2}) \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2} + \left(\frac{4 \alpha_1}{\alpha_4t^2}-1\right)\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2})\\
    \leq & \alpha_4t^4 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2} + \frac{4\alpha_1}{\alpha_4t^2}\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2})^. \end{split}
\end{align}
Next, we bound
\begin{align}\label{eq:inequality_tailbound2}
\begin{split}
    &\alpha_3 t^4 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2} \|_F^2 + 6\alpha_2 t^2 \langle \bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}\bm{\Sigma}_2^{1/2},\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\rangle\\
    \leq & \alpha_3 t^4 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2} \|_F^2 + 6\alpha_2 t^2 \langle \bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2},\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\rangle\\
    = & \langle \bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}, \alpha_3 t^4\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}+ 6 \alpha_2 t^2\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\rangle\\
    \leq & \alpha_3 t^4 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2} + \frac{6\alpha_2}{\alpha_3 t^2}\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\|_F\\
    \leq & \alpha_3 t^4 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2} + \frac{6\alpha_2}{\alpha_3 t^2}\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\|_F^2 \\
    \leq & \alpha_3 t^4 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2} + \frac{6\alpha_2}{\alpha_3 t^2}\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\|_F\\
    \leq & \alpha_3 t^4 \left(\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F + \frac{6\alpha_2}{\alpha_3 t^2}\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\|_F\right)^2, \end{split}
\end{align}
where the first inequality is due to \cite[Lemma 3.1 (i)]{persson2022randomized} and Lemma~\ref{lemma:loewner}, the second inequality is due to the Cauchy-Schwartz inuequality, the third inequality is due to \cite[Lemma 3.1 (i)]{persson2022randomized}, and the fourth inequality is due to the subadditivity of the square-root. 
Using the derived inequalities \eqref{eq:inequality_tailbound1} and \eqref{eq:inequality_tailbound2} and the subadditivity of the square-root we obtain
\begin{align*}
    U_t^2 &\leq \left(\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\|_F + \sqrt{\alpha_3} t^2 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2} + \frac{6\alpha_2}{\alpha_3 t^2}\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\|_F\right.\\
    + & \left. \sqrt{\alpha_4} t^2 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}) + \frac{4\alpha_1}{\sqrt{\alpha_4}} \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2})\right)\|\bm{K}_{11}^{-1}\|_2\\
    \leq & \left(\sqrt{\alpha_3} t^2 \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F + \left(1+ \frac{6\alpha_2}{\sqrt{\alpha_3}}\right)\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2}\|_F\right.\\
    + & \left.\sqrt{\alpha_4} t^2 \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}) + \frac{4\alpha_1}{\sqrt{\alpha_4}} \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}\bm{\Sigma}_2^{1/2})\right) \|\widetilde{\bm{K}}_{11}^{-1}\|_2,
\end{align*}
as required. 

\end{proof}
%Nicer version.
%\begin{theorem}
%Assume that $p = k \geq 4$ and $u ,t > 1$. Then with probability $1-3t^{-k} - e^{-u^2/2}$ we have
%\begin{align*}
    %&\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F + 2t^2\left(15 + \frac{4e^4}{k}\right)^{1/2}\|\widetilde{\bm{K}}_{11}^{-1}\|_2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F + 2\|\bm{\Sigma}_2\|_F\|\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_2^2\\
    %+ & 2t^2 \sqrt{\frac{4e^4 + 8 e^2}{k}} \|\widetilde{\bm{K}}_{11}^{-1}\|_2\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_* + \frac{4e^2}{k} \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_2 \|\widetilde{\bm{K}}_{11}^{-1}\|_2 t^2 u^2.
%\end{align*}
%Furthermore, if we define
%\begin{equation*}
    %\beta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \xi \in \{2,F,*\},
%\end{equation*}
%and
%\begin{equation*}
 %   \gamma_k = \frac{1}{\lambda_1 \|\bm{\widetilde{\bm{K}}}_{11}^{-1}\|_2},
%\end{equation*}
%then we have with probability at least $1-4t^{-p} - e^{-u^2/2}$
%\begin{align*}
 %   &\|\bm{A}-\widehat{\bm{A}}\|_F \leq \left(1 + O(1) \frac{\beta_k^{(F)}}{\gamma_k}t^2 + \|\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_2^2\right)\|\bm{\Sigma}_2\|_F + O\left(\frac{1}{\sqrt{k}}\right)\frac{\beta_k^{(*)}}{\gamma_k}t^2\|\bm{\Sigma}_2\|_* \\
    %+ & O\left(\frac{1}{k}\right) \frac{\beta_k^{(2)}}{\gamma_k}t^2u^2\|\bm{\Sigma}_2\|_2
%\end{align*}
%\end{theorem}
%\begin{remark}
%The hidden quantities are $(15 + \frac{4e^4}{k})^{1/2}, \sqrt{\frac{4e^4 + 8e^2}{k}}$ and $\frac{4e^2}{k}$.
%\end{remark}
%\begin{remark}
%The bound above states that if the covariance matrix is chosen perfectly (e.g. the orthogonal projection onto the range of the dominant singular vectors), then $\|\bm{A}-\widehat{\bm{A}}\|_F\leq \|\bm{\Sigma}_2\|_F$ with high probability, which matches with what would happen in reality. Furthermore, the terms $\beta_k^{(\xi)}$ together with $\gamma_k$ measure the quality of the covariance matrix. When $\bm{K} = \bm{I}$ we have $\beta_k^{(\xi)} = \gamma_k = 1$. In addition, $\|\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_2^2$ measures the dependence between $\bm{\Omega}_2$ and $\bm{\Omega_1}$. However, I am doubting whether it makes sense to include it. You can hide this term into the $O(1)$ constant above. Since the bounds for the Nyström approximation are not as clean as randomized SVD, I believe that we might not need to capture the case $\bm{K} = \bm{I}$ exactly anyway, but just capture the behaviour when $\bm{K} = \bm{I}$. 
%\end{remark}
%\begin{proof}
%It is clear that the second statement follows from the first statement. So it suffices to show the second statement. It follows immediately from bounding all the terms from Theorem~\ref{theorem:nystrom_tailbound1}. We $p = k$ we have 
%\begin{align*}
    %&\frac{4e^2}{(k+1)^2} \|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22.1}^{1/2}\|_2^2\|\widetilde{\bm{K}}_{11}^{-1}\|_2 \leq \frac{4e^2}{k}\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_2\|\widetilde{\bm{K}}_{11}^{-1}\|_2;\\
    %& \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 \leq \|\bm{\Sigma}_2\|_F^2\|\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_2^4;\\
    %& \|\bm{\Sigma}_2^{1/2} \bm{K}_{22.1}^{1/2}\|_{(4)}^4 \left(\frac{9 \tr(\widetilde{\bm{K}}_{11}^{-1})^2}{(k+1)^2} + \frac{4e^4 \|\widetilde{\bm{K}}_{11}^{-1}\|_F^2 k^2}{(k+1)^4}\right) \leq \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2(9 + \frac{4e^4}{k})\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2\\
    %& \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_F^4 \frac{4e^4\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2k^2}{(k+1)^4} \leq \tr(\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})^2 \frac{4e^4}{k} \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2;\\
    %& \frac{6}{k+1}\|\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2 \tr(\widetilde{\bm{K}}_{11}^{-1}) \leq 6\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_F^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_2^2;\\
    %&8e^2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_F^2 \frac{k \|\widetilde{\bm{K}}_{11}^{-1}\|_2}{(k+1)^2} \leq \frac{8e^2\|\widetilde{\bm{K}}_{11}^{-1}\|_2^2}{k}\tr(\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2})^2.
%\end{align*}
%Inserting the obtain inequalities into the tailbound and the subadditivity of the square-root yields the result. 
%\end{proof}


==> Notes/finitedim_rsvd.tex <==
\section{The finite dimensional randomized SVD}

\subsection{Structural bound}
By Lemma~\ref{lemma:partition} $\bm{\Omega}_1$ is distributed as $N(\bm{0}, \widetilde{\bm{K}}_{11})$ and therefore has full rank since we assumed $\rank(\widetilde{\bm{K}}_{11}) = k$\footnote{To see this note that $\bm{\Omega}_1 = \widetilde{\bm{K}}_{11}^{1/2} \bm{X}$ where $\bm{X}$ is a standard Gaussian matrix. Then, $\bm{\Omega}_1\bm{\Omega}_1^T = \widetilde{\bm{K}}_{11}^{1/2} \bm{X}\bm{X}^T \widetilde{\bm{K}}_{11}^{1/2}$ is full-rank a.s. since $\bm{X}\bm{X}^T$ is full-rank a.s. }. Therefore, we have the following lemma.
\begin{lemma}[{\cite[Theorem 9.1]{rsvd}}]\label{lemma:structural_bound}
Let $\bm{Q}$ be an orthonormal basis for $\range(\bm{A\Omega})$. Then, if $\bm{\Omega}_1$ has full row-rank we have
\begin{equation*}
    \|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_{2,F}^2 \leq \|\bm{\Sigma}_2\|_{2,F}^2 + \|\bm{\Sigma}_2\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{2,F}^2.
\end{equation*}
\end{lemma}
\subsection{Expectation bound}
Useful imported lemmas from \cite[Theorem 5.1]{multstat}, \cite[Theorem 5.3]{multstat}, and \cite[Theorem 2.4.14]{kollo}.
\begin{lemma}\label{lemma:gaussian_facts}
Consider
\begin{equation*}
    \begin{bmatrix} \bm{\Omega}_1 \\ \bm{\Omega}_2 \end{bmatrix} \sim N\left(\bm{0},\begin{bmatrix} \widetilde{\bm{K}}_{11}  & \widetilde{\bm{K}}_{21}^T \\ \widetilde{\bm{K}}_{21} & \widetilde{\bm{K}}_{22} \end{bmatrix}\right).
\end{equation*}.
Then,
\begin{enumerate}
    \item $\bm{\Omega}_1 \sim N(\bm{0},\widetilde{\bm{K}}_{11})$; \label{lemma:partition}
    \item $\bm{\Omega}_2 | \bm{\Omega}_1 \sim N(\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} \bm{\Omega}_1, \widetilde{\bm{K}}_{22}-\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T)$; \label{lemma:cond_distribution}\\
    \item $\bm{\Omega}_1 \bm{\Omega}_1^T \sim \mathcal{W}_{k}(\widetilde{\bm{K}}_{11},k+p)$, $(\bm{\Omega}_1\bm{\Omega}_1^T)^{-1} \sim \mathcal{W}^{-1}_k(\widetilde{\bm{K}}_{11}^{-1},k+p)$, and
    \begin{equation*}
    \mathbb{E}[(\bm{\Omega}_1\bm{\Omega}_1^T)^{-1}] = \frac{\widetilde{\bm{K}}_{11}^{-1}}{p-1}. \label{lemma:inversewishart_expectation}
    \end{equation*}
\end{enumerate}
\end{lemma}
\quad\\
Prepatory lemma.
\begin{lemma}\label{lemma:frobeniusinverse_expectation}
If $p \geq 2$
\begin{equation*}
    \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_F^2 = \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}.
\end{equation*}
\end{lemma}
\begin{proof}
Note that since $\bm{\Omega}_1$ has full row rank, then
\begin{equation*}
    \bm{\Omega}_1^{\dagger} = \bm{\Omega}_1^T(\bm{\Omega}_1\bm{\Omega}_1^T)^{-1}.
\end{equation*}
Hence,
\begin{equation*}
    \|\bm{\Omega}_1^{\dagger}\|_F^2 = \tr((\bm{\Omega}_1\bm{\Omega}_1^T)^{-1}).
\end{equation*}
Furthermore, by Lemma~\ref{lemma:gaussian_facts}~(\ref{lemma:inversewishart_expectation}) and the linearity of the trace we have%Lemma~\ref{lemma:inversewishart_expectation}
\begin{equation*}
    \mathbb{E} \tr((\bm{\Omega}_1\bm{\Omega}_1^T)^{-1}) = \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1},
\end{equation*}
as required.
\end{proof}
\quad\\
Main result.
\begin{theorem}\label{theorem:frobenius_expectation_bound1}
If $p \geq 2$, then
\begin{equation*}
    \mathbb{E}\|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_F^2 \leq \|\bm{\Sigma}_2\|_F^2 + \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 - \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1/2}\|_F^2 \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} + \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22} \bm{\Sigma}_2)\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}.
\end{equation*}
\end{theorem}
\begin{proof}
By Lemma~\ref{lemma:gaussian_facts}~(\ref{lemma:cond_distribution}), it suffices to bound $\mathbb{E}\|\bm{\Sigma}_2 \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_F^2$. Let $\bm{\Psi}$ be a standard Gaussian matrix of size $(n-k)\times (k+p)$. Then, using Lemma~\ref{lemma:gaussian_facts}~(\ref{lemma:cond_distribution}) we have
\begin{equation*}
    \bm{\Omega}_2|\bm{\Omega}_1 \sim \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} \bm{\Omega}_1 + \widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Psi}.
\end{equation*}
Hence,
\begin{align*}
    &\mathbb{E}\|\bm{\Sigma}_2 \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_F^2 = \mathbb{E}[\mathbb{E}[\|\bm{\Sigma}_2 \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_F^2|\bm{\Omega}_1]] =  \mathbb{E}[\mathbb{E}[\bm{\Sigma}_2 (\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} \bm{\Omega}_1 + \widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Psi})\bm{\Omega}_1^{\dagger}|\bm{\Omega}_1]]\\
    = & \mathbb{E}[\mathbb{E}[\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1} + \bm{\Sigma}_2\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Psi}\bm{\Omega}_1^{\dagger}|\bm{\Omega}_1]]\\
    = & \mathbb{E}[\mathbb{E}[ \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 + \|\bm{\Sigma}_2\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Psi}\bm{\Omega}_1^{\dagger}\|_F^2 + 2\tr(\bm{\Sigma}_2\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Psi}\bm{\Omega}_1^{\dagger}(\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1})^T)|\bm{\Omega}_1]]\\
    = &\|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 + \mathbb{E}[\mathbb{E}[\|\bm{\Sigma}_2\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Psi}\bm{\Omega}_1^{\dagger}\|_F^2|\bm{\Omega}_1]] = \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 + \|\bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2 \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_F^2\\
    = & \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 + \|\bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2 \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1},
\end{align*}
where we used \cite[Proposition 10.1]{rsvd}, Lemma~\ref{lemma:frobeniusinverse_expectation}, and 
\begin{equation*}
    \mathbb{E}[\mathbb{E}[\tr(\bm{\Sigma}_2\widetilde{\bm{K}}_{22.1} \bm{\Psi}\bm{\Omega}_1^{\dagger}(\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1})^T)|\bm{\Omega}_1]] = 0,
\end{equation*}
To obtain the final result we note that 
\begin{align*}
    &\|\bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2 \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} = \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1} \bm{\Sigma}_2) \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}\\
    = & - \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}^{-1}_{11}\widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2)\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} + \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22} \bm{\Sigma}_2)\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}\\
    = & - \|\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}^{-1/2}_{11}\|_F^2\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} + \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22} \bm{\Sigma}_2)\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}
\end{align*}
\end{proof}
\quad\\
We can simplify \cref{theorem:frobenius_expectation_bound1} as follows:
\begin{corollary}\label{corollary:expectation_bound_rsvd}
Let $\lambda_1 = \|\bm{K}\|_2 = \|\widetilde{\bm{K}}\|_2$, and
\begin{equation*}
    \beta_k = \frac{\tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22}\bm{\Sigma}_2)}{\lambda_1 \|\bm{\Sigma}_2\|_F^2}, \quad \delta_k = \frac{\tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}\bm{\Sigma}_2)}{\lambda_1 \|\bm{\Sigma}_2\|_F^2}, \quad\gamma_k = \frac{k}{\lambda_1 \tr(\widetilde{\bm{K}}_{11}^{-1})}.
\end{equation*}
If $p \geq 2$, then
\[\mathbb{E}\|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_F^2\leq \left(1+\frac{k}{p-1}\frac{\beta_k}{\gamma_k}+k\frac{\delta_k}{\gamma_k}\right)\|\bm{\Sigma}_2\|_F^2.\]
\end{corollary}

\begin{remark}
The first term in the sum is the best approximation error, the second term is the standard randomized SVD error from \cite[Theorem 10.5]{rsvd}, the last term measures the independence between $\bm{\Omega}_1$ and $\bm{\Omega}_2$. The second term measures how well $\bm{K}$ points in the direction of the optimal singular subspace of $\bm{A}$. Furthermore, note that $\widetilde{\bm{K}}_{22} \succeq \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T \succeq 0$. In the ideal scenario, $\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T = 0$, which holds if and only if $\bm{\Omega}_1$ is independent of $\bm{\Omega}_2$. Furthermore, in the worst scenario $\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1} \widetilde{\bm{K}}_{21}^T = \widetilde{\bm{K}}_{22}$, which holds if and only if $\bm{\Omega}_2$ is completely determined by $\bm{\Omega}_1$. Hence, we want to choose $\bm{K}$ such that both $\beta_k$ and $\delta_k$ are close to 0. However, since the Schur complement is positive semi-definite it is not difficult to see that $\beta_k \geq \delta_k$. Additionally, if we have a good approximation of the first $k$ right singular vectors of $\bm{A}$, we can tune the covariance matrix to have strong eigenvalue $\lambda_j$ decay for $j>k$, which would drive $\beta_k$ to $0$.
\end{remark}

\begin{proof}
By submultiplicativity of the Frobenius norm, we have
\begin{equation*}
    \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_F^2\leq \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11} \widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2)\tr(\widetilde{\bm{K}}^{-1}_{11})
\end{equation*}
%\[
%\|\bm{\Sigma}_2\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_F^2\leq
%\|\bm{\Sigma}_2\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1/2}\|_2^2 \tr(\widetilde{\bm{K}}_{11}^{-1}).
%\]
Then, by applying Theorem~\ref{theorem:frobenius_expectation_bound1} and omitting any negative terms we obtain
\begin{align*}
    \mathbb{E}\|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_F^2 &\leq \|\bm{\Sigma}_2\|_F^2 + \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 + \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22} \bm{\Sigma}_2)\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}.\\
    &\leq \left(1+\frac{k}{p-1}\frac{\beta_k}{\gamma_k}+k \frac{\delta_k}{\gamma_k}\right)\|\bm{\Sigma}_2\|_F^2,
\end{align*}
as required.
\end{proof}

\begin{remark}
If we let $\bm{K} = (\bm{A}^T \bm{A})^{2q} = \bm{V} \bm{\Sigma}^{4q}\bm{V}^T$, which corresponds to the performing subspace iteration, we obtain,
\begin{align*}
    &\|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_{2,F}^2 \leq \|\bm{\Sigma}_2\|_{F}^2 + \frac{\|\bm{\Sigma}_2^{2q+1}\|_F^2 \|\bm{\Sigma}_1^{-2q}\|_F^2}{p-1} \\
    \leq & \left(1+\left(\frac{\sigma_{k+1}}{\sigma_k}\right)^{4q} \frac{k}{p-1}\right)\|\bm{\Sigma}_2\|_F^2.
\end{align*}
\end{remark}
\quad\\
We can show that Lemma~\ref{theorem:frobenius_expectation_bound1} is tighter than \cite[Proposition 6]{boulle2021a}.
\begin{corollary}
In the setting of Corollary~\ref{corollary:expectation_bound_rsvd}. Then,
\begin{equation*}
    \mathbb{E}\|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_F^2 \leq \left(1+k \frac{\beta_k}{\gamma_k}\right)\|\bm{\Sigma}_2\|_F^2.
\end{equation*}
\end{corollary}
\begin{remark}
This improves on \cite[Proposition 6]{boulle2021a}, since it removes the $\frac{k+p}{p-1} > 1$ constant. However, if we use standard Gaussians we have $\beta_k = \gamma_k =1$, and we don't recover \cite[Theorem 10.5]{rsvd}. 
\end{remark}
\begin{proof}
Note that it suffices to bound
\begin{equation*}
    \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 - \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1/2}\|_F^2\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} \leq \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22} \bm{\Sigma}_2)\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} (p-2),
\end{equation*}
because then we would have
\begin{align*}
    &\|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 - \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1/2}\|_F^2 \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} + \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22} \bm{\Sigma}_2)\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}\\
    \leq & \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22} \bm{\Sigma}_2) \tr(\widetilde{\bm{K}}_{11}) = k\frac{\beta_k}{\gamma_k}\|\bm{\Sigma}_2\|_F^2.
\end{align*}
Using submultiplicativity and that the Schur complement $\widetilde{\bm{K}}_{22} - \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T$ is symmetric positive semi-definite, we have
\begin{align*}
    &\|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 - \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1/2}\|_F^2\frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}\\
    \leq & \|\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1/2}\|_F^2 \tr(\widetilde{\bm{K}}_{11}^{-1})(1-\frac{1}{p-1}) = \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2) \tr(\widetilde{\bm{K}}_{11}^{-1}) \frac{p-2}{p-1}\\
    \leq & \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22}\bm{\Sigma}_2)\tr(\widetilde{\bm{K}}_{11}^{-1}) \frac{p-2}{p-1},
\end{align*}
as required.
\end{proof}

\subsection{Deviation bounds}

%Using \cref{lemma:cond_distribution}, we know that 
%\[\Omega_2|\Omega_1\sim \mathcal{N}(m,C),\]
%where $m=\widetilde{K}_{21}\widetilde{K}_{11}^{-1}\Omega_1$ and $C=\widetilde{K}_{22}-\widetilde{K}_{11}^{-1}\widetilde{K}_{21}^T$. Moreover, we have the following result for concentration of functions of a Gaussian matrix~\cite[Prop.~10.3]{rsvd}:
Prepatory lemma.
\begin{lemma}[{\cite[Proposition 10.3]{rsvd}}] \label{prop_proba_lip}
Suppose that $h$ is a Lipschitz function on matrices satisfying
\[|h(\bm{X})-h(\bm{Y})|\leq L\|\bm{X}-\bm{Y}\|_F,\quad \forall \bm{X},\bm{Y}.\]
Draw a standard Gaussian matrix $G$, then
\[\mathbb{P}\left\{h(\bm{G})\geq \mathbb{E}h(\bm{G})+Lt\right\}\leq e^{-t^2/2}.\]
\end{lemma}
\quad\\
Prepatory lemma.
\begin{lemma}\label{lemma:tailbound_shifted_pnorm}
Let $\bm{B}, \bm{C}$ and $\bm{D}$ be fixed matrices, and $\bm{\Psi}$ and standard Gaussian matrix. Then, for $s \geq 2$ we have
\begin{equation*}
    \mathbb{P}\left(\|\bm{B}+\bm{C}\bm{\Psi}\bm{D}\|_{(s)} \geq \mathbb{E}\|\bm{B}+\bm{C}\bm{\Psi}\bm{D}\|_{(s)} + \|\bm{C}\|_2 \|\bm{D}\|_2 u\right) \leq e^{-u^2/2}.
\end{equation*}
\end{lemma}
\begin{proof}
It suffices to show that $h(\bm{X}) = \|\bm{B}+\bm{C}\bm{X}\bm{D}\|_{(s)}$ is Lipschitz continuous with Lipschitz constant $\|\bm{C}\|_2 \|\bm{D}\|_2$. The final result is obtained by applying Lemma~\ref{prop_proba_lip}. We have by the triangle inequality
\begin{equation*}
    |h(\bm{X})-h(\bm{Y})| \leq \|\bm{C}(\bm{X}-\bm{Y})\bm{D}\|_{(s)} \leq \|\bm{C}\|_2 \|\bm{D}\|_2\|\bm{X}-\bm{Y}\|_{(s)} \leq \|\bm{C}\|_2 \|\bm{D}\|_2\|\bm{X}-\bm{Y}\|_{F},
\end{equation*}
where we used that the Frobenius norm is larger than any Schatten-$s$ norm for $s \geq 2$.
\end{proof}
\quad\\
Main theorem.
\begin{theorem}
Assume that $p \geq 4$ and $u,t >1$. Then with probability at least $1-2t^{-p} - e^{-u^2/2}$ we have
\begin{equation*}
    \|(\bm{I}-\bm{Q}\bm{Q}^T)\bm{A}\|_F \leq \left(1 + \sqrt{t^2\frac{3k}{p+1} \frac{\beta_k}{\gamma_k} + k \frac{\delta_k}{\gamma_k}}\right)\|\bm{\Sigma}_2\|_F + ut \frac{e\sqrt{k+p}}{p+1}\|\bm{\Sigma}_2\widetilde{\bm{K}}_{22.1}^{1/2}\|_2 \sqrt{\|\widetilde{\bm{K}}_{11}^{-1}\|_2}.
\end{equation*}
\end{theorem}
\begin{proof}
The proof is identical to \cite[Theorem 10.7]{rsvd}, utilizing Lemma~\ref{prop_proba_lip}, Theorem~\ref{theorem:frobenius_expectation_bound1} and Lemma~\ref{lemma:omega1_tailbound}.
\end{proof}

\begin{remark}
\textcolor{red}{The theorem should probably be simplified even further, but there is no rush in doing that now. We should say for example that $\|\bm{\Sigma}_2\widetilde{\bm{K}}_{22.1}^{1/2}\|_2 \leq \sqrt{\|\bm{\Sigma}_2 \widetilde{\bm{K}}_{22} \bm{\Sigma}_2\|_2}$.}
\end{remark}

Following the proof of~\cite[Prop.~10.7]{rsvd}, after conditioning on $\Omega_1$, we need to get a probability bound for the quantity $\|\Sigma_2\Omega_2\Omega_1^\dagger\|_F$. We first note that $\Omega_2 \sim m + C^{1/2}X$, where $X$ is standard Gaussian. Consider the function $h(X)=\|\Sigma_2(m+C^{1/2}X)\Omega_1^\dagger\|_F$, then by the triangular inequality
\[|h(X)-h(Y)|\leq \|\Sigma_2 C^{1/2}(X-Y)\Omega_1^\dagger\|_F\leq \|\Sigma_2 C^{1/2}\|_F\|\Omega_1^\dagger\|_F\|X-Y\|_F,\]
where the last inequality comes from the submultiplicativity of the Frobenius norm. Therefore, $h$ is Lipschitz with Lipschitz constant $L = \|\Sigma_2 C^{1/2}\|_F\|\Omega_1^\dagger\|_F$. Applying \cref{prop_proba_lip} on the standard Gaussian matrix $X$ gives
\[\mathbb{P}\left\{\|\Sigma_2\Omega_2\Omega_1^\dagger\|_F\geq \mathbb{E}[\|\Sigma_2\Omega_2\Omega_1^\dagger\|_F]+\|\Sigma_2 C^{1/2}\|_F\|\Omega_1^\dagger\|_Ft\right\}\leq e^{-t^2/2}.\]

To extend the result to infinite dimension, we first denote $\Sigma_2^{(n)}$ and $\Omega_2^{(n)}$ the truncation of $\Sigma_2$ and $\Omega_2$ to the first $n$ rows for $n\geq 1.$ Let $C_n$ be the covariance matrix of $\Omega_2^{(n)}$ such that $\|\Sigma_2^{(n)}C^{(1/2)}_n\|_{HS}\to_{n\to\infty} \|\Sigma_2 C^{1/2}\|_{HS}$ \textcolor{red}{Here $C$ is an infinite matrix?}. We want to show that
\begin{align*}
\lim_{n\to\infty} & \mathbb{P}\left\{\|\Sigma_2^{(n)}\Omega_2^{(n)}\Omega_1^\dagger\|_F\geq \mathbb{E}[\|\Sigma_2^{(n)}\Omega_2^{(n)}\Omega_1^\dagger\|_F]+\|\Sigma_2 C_n^{1/2}\|_F\|\Omega_1^\dagger\|_Ft\right\}\\
&=\mathbb{P}\left\{\|\Sigma_2\Omega_2\Omega_1^\dagger\|_F\geq \mathbb{E}[\|\Sigma_2\Omega_2\Omega_1^\dagger\|_F]+\|\Sigma_2 C^{1/2}\|_F\|\Omega_1^\dagger\|_Ft\right\}.
\end{align*}

\begin{proposition} \label{prop_convergence_Omega}
Let $\Omega_2=\begin{pmatrix}
\omega_1 & \ldots &\omega_k
\end{pmatrix}\in \mathbb{R}^{\mathbb{N}\times k}$ be a quasimatrix whose columns are i.i.d. sampled from a Gaussian process with mean zero and compact covariance operator $C:\ell_2\times\ell_2\to\mathbb{R}$ of trace class. Let $n\geq 1$ be a nonzero integer and consider the truncation $\Omega_2^{(n)}$ of $\Omega_2$ to the $n$th entry. Then $\|\Omega_2^{(n)}\|_{HS}$ converges in probability to $\|\Omega_2\|_{HS}$.
\end{proposition}

{\color{blue} Maybe the formulation of \cref{prop_convergence_Omega} is not super rigorous due to the truncation of $\Omega_2$ not well defined. What we should do instead is get a proposition that directly shows an infinite dimensional analogue of \cref{prop_proba_lip}. Then say: by Karhunen-Loeve theorem, there exists an orthonormal eigenbasis $\{\psi_i,\lambda_i\}$ such that $\omega_j\sim \ldots$, now consider the truncation to the $n$th entry, and show convergence. I'm leaving this for the final write-up.}

\begin{proof}
Let $\{\psi_i,\lambda_i\}_{i\in \mathbb{N}_{\geq 1}}$ be the orthonormal eigenfunctions and eigenvalues of $C$ such that
\[\omega_j\sim \sum_{i=1}^\infty \sqrt{\lambda_i} c_i^{(j)} \psi_i,\quad 1\leq j\leq k,\]
where $\omega_j\in \ell_2$ with probability one. Let $n\geq 1$, then, $\omega_j^{(n)}$ is defined as follows:
\[\omega_j^{(n)}(i) = 
\begin{cases}
\omega_j(i) & \text{if } i\leq n,\\
0 & \text{otherwise}.
\end{cases}
\]
Hence, $\Omega_2^{(n)}$ follows a multivariate normal distribution with mean zero and covariance matrix $C_n\in \mathbb{R}^{n\times n}$ in the finite dimensional space spanned by $\psi_1,\ldots,\psi_n$ \textcolor{red}{I don't quite understand this. The covariance matrix of the columns in $\Omega_2^{(n)}$ is $C(1:n, 1:n)$ (padded with a bunch of zeros after this block). Hence, each column of $\Omega_2^{(n)}$ falls in the range of $C(1:n, 1:n)$. Why would $\psi_1,\ldots,\psi_n$ span this space? This would require that $\range(C(1:n,1:n)) = \text{span}\{e_1,\ldots,e_n\} = \text{span}\{\psi_1,\ldots,\psi_n\}$, where $e_i$ is the $i^{\text{th}}$ canonical vector.}\\\\
\textcolor{red}{Are you actually saying that $\omega_j^{(n)} = \sum\limits_{i=1}^n \sqrt{\lambda_i} c_i^{(j)} \psi_i$? (Truncating the series rather than the entries) Because then I would agree, and the rest of your argument makes sense to me. However, the next problem for me would be that I don't see exactly how this will help us to extend the bounds for the rSVD to infinite dimensions.}. By the continuous mapping theorem, we can prove that the real random variable $X_n=\|\Omega_2^{(n)}\|_{HS}^2$ converges in probability to $X=\|\Omega_2\|_{HS}^2$. Let $\epsilon>0$, we want to show that the following equality holds:
\[\lim_{n\to\infty}\mathbb{P}(|X-X_n|>\epsilon)=0.\]
Let $n\geq 1$, since $|X-X_n|$ is a nonnegative random variable, Markov inequality yields
\[\mathbb{P}(|X-X_n|>\epsilon)\leq \frac{\mathbb{E}(|X-X_n|)}{\epsilon}.\]
Then,
\[\|\Omega_2^{(n)}\|_{HS}^2 = \sum_{j=1}^k\langle \omega_j^{(n)},\omega_j^{(n)}\rangle=\sum_{i=1}^n \lambda_i\sum_{j=1}^k [c_i^{(j)}]^2,\]
and
\[|X-X_n| = \sum_{i=n+1}^\infty \lambda_i\sum_{j=1}^k [c_i^{(j)}]^2.\]
Applying Fubini-Tonelli theorem gives,
\[E(|X-X_n|) \leq \sum_{i=n+1}^\infty \lambda_i\sum_{j=1}^k V([c_i^{(j)}]^2).\]
However, the $[c_i^{(j)}]^2\sim \chi^2$, hence $E([c_i^{(j)}]^2)=1$, which gives
\[E(|X-X_n|)\leq k\sum_{i=n+1}^\infty \lambda_i\to 0,\]
since $\sum_{i=1}^\infty \lambda_i=\tr(C)<\infty$. This achieves the proof that $\|\Omega_2^{(n)}\|_{HS}$ converges to $\|\Omega_2\|_{HS}$ in probability. 
\end{proof}

\begin{remark}
Note that the generalization to $\|\Sigma_2^{(n)}\Omega_2^{(n)}\Omega_1^\dagger\|_F$ is trivial since
\[\|\Sigma_2^{(n)}\Omega_2^{(n)}\Omega_1^\dagger\|_F\leq \|\Sigma_2\|_F\|\Omega_2^{(n)}\|_F\|\Omega_1^\dagger\|_F,\]
by submultiplicativity of the HS norm, which shows convergence of $\|\Sigma_2^{(n)}\Omega_2^{(n)}\Omega_1^\dagger\|_F$ in probability.
\end{remark}

\begin{corollary}
\begin{align*}
\lim_{n\to\infty} & \mathbb{P}\left\{\|\Omega_2^{(n)}\|_{HS}\geq \mathbb{E}[\|\Omega_2^{(n)}\|_{HS}]+\|C_n^{1/2}\|_{HS} t\right\}\\
&=\mathbb{P}\left\{\|\Omega_2\|_{HS}\geq \mathbb{E}[\|\Omega_2\|_F]+\|C^{1/2}\|_{HS} t\right\},
\end{align*}
\end{corollary}

\textcolor{red}{I am convinced of the convergence of $\|\Omega_2^{(n)}\|_F$ to $\|\Omega_2\|_F$, but I don't see how the final argument implies the convergence of $\|\Sigma_2^{(n)}\Omega_2^{(n)} \Omega_1^{\dagger}\|_F$ to  $\|\Sigma_2\Omega_2 \Omega_1^{\dagger}\|_F$}

{\color{red}I add an alternate proof of the convergence of $\|\Omega_2^{(n)}\|_F$ to $\|\Omega_2\|_F$ here, which might even be exactly what you wrote above. I still add it for my own understanding. We need to show that $\mathbb{E}|X-X_n| = \mathbb{E}[\|\Omega_2\|_F - \|\Omega_2^{(n)}\|_F]$ converges to zero. By triangle inequality
\begin{equation*}
    X-X_n \leq \|\Omega_2 - \Omega_2^{(n)}\|_F  \leq \sum\limits_{j=1}^k \|\omega_j-\omega_j^{(n)}\|_2,
\end{equation*}
where $\omega_j^{(n)}$ is defined as follows:
\[\omega_j^{(n)}(i) = 
\begin{cases}
\omega_j(i) & \text{if } i\leq n,\\
0 & \text{otherwise}.
\end{cases}
\]
Hence, it is sufficient to show that $\mathbb{E}\|\omega_j - \omega_j^{(n)}\|_2$ converges to zero. For simplicity, drop the subscript from $\omega_j$ and $\omega_j^{(n)}$, so that we consider $\omega$ and $\omega^{(n)}$.Note that $\omega \in \mathbb{R}^{\infty}$ (an infinite vector, not a quasimatrix) and the $i^{\text{th}}$ entry equals
\begin{equation*}
    \omega(i) = \langle u_{i+k}, f\rangle = \sum\limits_{j=1}^{\infty} \sqrt{\lambda_j} \langle u_{i+k}, \psi_j \rangle c_j, \quad c_j \stackrel{iid}{\sim} N(0,1),
\end{equation*}where $f \sim GP(0,K)$, $\psi_j$ is the eigenvectors of $K$ (the eigenvectors are functions in $L^2$), and $u_j$ is the $j^{\text{th}}$ singular vector of the operator that we are approximating.\footnote{Here I am saying that $\omega = U_2^T f$, where $f$ is our sketch Gaussian process.} Consequently,
\begin{equation*}
    w(i) \sim N\left(0, \sum\limits_{j=1}^{\infty} \lambda_j \langle u_{i+k}, \psi_j \rangle^2\right)
\end{equation*}
It is clear that $\omega(i)$ has a finite variance, since $\tr(K) = \sum\limits_{i=1}^{\infty} \lambda_i < \infty$ and $\langle u_{i+k}, \psi_j\rangle^2 \leq 1$. For simplicity, write $\langle u_{i+k}, \psi_j \rangle = M(i,j)$
and
\begin{equation*}
    \sigma_i^2 = \sum\limits_{j=1}^{\infty} \lambda_j \langle u_{i+k}, \psi_j \rangle^2.
\end{equation*}
This implies that
\begin{equation*}
    \sum\limits_{i=1}^{\infty} \sigma_i^2 = \sum\limits_{i=1}^{\infty} \sum\limits_{j=1}^{\infty}\lambda_j M(i,j)^2 =\sum\limits_{j=1}^{\infty} \sum\limits_{i=1}^{\infty}\lambda_j M(i,j)^2.
\end{equation*}
Note that
\begin{equation*}
    \sum\limits_{i=1}^{\infty} M(i,j)^2 = \sum\limits_{i=1}^{\infty} \langle u_{i+k}, \psi_j \rangle^2 = \|U_2 U_2^T\psi_j\|_{L^2}^2 \leq \|\psi_j\|_{L^2}^2 = 1,
\end{equation*}
which implies that 
\begin{equation*}
    \sum\limits_{i=1}^{\infty} \sigma_i^2 \leq \sum\limits_{j=1}^{\infty} \lambda_j = \tr(K) < \infty.
\end{equation*}
Note that
\begin{equation*}
    \mathbb{E}\|\omega\|_2^2 = \sum\limits_{i=1}^{\infty} \mathbb{E}\omega(i)^2 = \sum\limits_{i=1}^{\infty} \sigma_i^2 < \infty.
\end{equation*}
Hence,
\begin{equation*}
    \mathbb{E}\|\omega-\omega^{(n)}\|_2 \leq \sqrt{\mathbb{E}\|\omega-\omega^{(n)}\|_2^2} = \sqrt{\sum\limits_{i=n+1}^{\infty} \mathbb{E}\omega(i)^2}= \sqrt{\sum\limits_{i=n+1}^{\infty} \sigma_i^2} \rightarrow_{n \rightarrow \infty} 0,
\end{equation*}
since $\sum\limits_{i=1}^{\infty} \sigma_i^2 < \infty$.}

In fact, for any $s \geq 2$ we have that ($\bm{\Omega}_1^{\dagger}$ is not fixed!)
\begin{align*}
    &\|\bm{\Sigma}_2^{2/s} \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(s)}-\|\bm{\Sigma}_2^{(n)2/s} \bm{\Omega}_2^{(n)} \bm{\Omega}_1^{\dagger}\|_{(s)} \leq \|\bm{\Sigma}_2^{2/s} \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}-\bm{\Sigma}_2^{(n)2/s} \bm{\Omega}_2^{(n)} \bm{\Omega}_1^{\dagger}\|_{(s)}\\
    = & \|\bm{\Sigma}_2^{2/s} \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}-\bm{\Sigma}_2^{2/s} \bm{\Omega}_2^{(n)} \bm{\Omega}_1^{\dagger}\|_{(s)} \leq \|\bm{\Sigma}_2\|_F^{2/s} \|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{(s)} \|\bm{\Omega}_1^{\dagger}\|_2 \\
    \leq & \|\bm{\Sigma}_2\|_F^{2/s} \|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{F} \|\bm{\Omega}_1^{\dagger}\|_2 \stackrel{d}{\rightarrow} 0,
\end{align*}
where in the first equality we can remove the superscript $(n)$ and the final limit follows from the product rule of convergence of random variables (since one of them converges to a constant). So I guess that any tailbound that we would have for $\|\bm{\Sigma}_2^{(n)2/s} \bm{\Omega}_2^{(n)} \bm{\Omega}_1^{\dagger}\|_{(s)}$ would immediately hold for $\|\bm{\Sigma}_2^{2/s} \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(s)}$. I.e. if we let $X_n = \|\bm{\Sigma}_2^{(n)2/s} \bm{\Omega}_2^{(n)} \bm{\Omega}_1^{\dagger}\|_{(s)}$ and $X = \|\bm{\Sigma}_2^{2/s} \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(s)}$, then if 
\begin{equation*}
    \mathbb{P}(X_n \geq x_n) \leq T
\end{equation*}
where $T$ is fixed and $x_n \rightarrow x$, then
\begin{equation*}
    \mathbb{P}(X \geq x) \leq T.
\end{equation*}
So we don't need to condition on $\Omega_1$ first when we deal with the infinite-dimensional case, we just need to show that $x_n \rightarrow x$. 

==> Notes/finitedim_setting.tex <==
\section{The finite dimensional setting}
Consider a matrix $\bm{A} \in \mathbb{R}^{m \times n}$ with SVD
\begin{equation*}
    \bm{A} = \bm{U} \bm{\Sigma} \bm{V}^T = \begin{bmatrix} \bm{U}_1 & \bm{U}_2 \end{bmatrix} \begin{bmatrix} \bm{\Sigma}_1 & \\ & \bm{\Sigma}_2 \end{bmatrix} \begin{bmatrix} \bm{V}_1^T \\ \bm{V}_2^T \end{bmatrix}.
\end{equation*}
where $\bm{U}_1 \in \mathbb{R}^{m \times k}, \bm{\Sigma}_1 \in \mathbb{R}^{k \times k}$ and $\bm{V}_1 \in \mathbb{R}^{n \times k}$. Let $\bm{K} \in \mathbb{R}^{n \times n}$ be an arbitrary symmetric positive semi-definite matrix. Let 
\begin{equation*}
    \widetilde{\bm{K}} = \bm{V}^T \bm{K} \bm{V} = \begin{bmatrix} \bm{V}_1^T \bm{K} \bm{V}_1 & \bm{V}_1^T \bm{K} \bm{V}_2 \\ \bm{V}_2^T \bm{K} \bm{V}_1 & \bm{V}_2^T \bm{K} \bm{V}_2 \end{bmatrix} = \begin{bmatrix} \widetilde{\bm{K}}_{11} & \widetilde{\bm{K}}_{21}^T \\ \widetilde{\bm{K}}_{21} & \widetilde{\bm{K}}_{22} \end{bmatrix}.
\end{equation*}
We further assume that $\rank(\widetilde{\bm{K}}_{11}) = k$ and we denote $\widetilde{\bm{K}}_{22.1} = \widetilde{\bm{K}}_{22}-\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T$. Let $\bm{\Omega}$ is an $n \times (k+p)$ is a random matrix whose columns are i.i.d. samples from $N(\bm{0}, \bm{K})$, and denote
\begin{equation*}
    \bm{\Omega}_1 = \bm{V}_1^T \bm{\Omega}, \quad \bm{\Omega}_2 = \bm{V}_2^T \bm{\Omega}.
\end{equation*}


==> Notes/infdim_nystrom2.tex <==
\section{The infinite dimensional Nyström approximation}

\subsection{Structural bound}
\begin{lemma}
Let $\mathcal{A}$ be a symmetric trace class and assume that $\bm{\Omega}_1$ has full rank. Then,
\begin{equation*}
    \|\mathcal{A}- \mathcal{A} \Omega(\Omega^T\mathcal{A} \Omega)^{\dagger}(\mathcal{A}\Omega)^T\|_F \leq \|\bm{\Sigma}_2\|_F + \|\bm{\Sigma}_2 \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^2.
\end{equation*}
\end{lemma}
\begin{proof}
Let us define $\widetilde{\bm{\Omega}} = U^T \Omega$ and $UU^T$ be the orthogonal projection onto the range of $\mathcal{A}$. Since $\mathcal{A}$ is self-adjoint we have
\begin{equation*}
    \mathcal{A} = UU^T \mathcal{A} = \mathcal{A} UU^T = UU^T \mathcal{A} UU^T.
\end{equation*}
Thus,
\begin{align*}
    &\|\mathcal{A}- \mathcal{A} \Omega(\Omega^T\mathcal{A} \Omega)^{\dagger}(\mathcal{A}\Omega)^T\|_F = \|UU^T\mathcal{A}UU^T- UU^T\mathcal{A}UU^T \Omega(\Omega^TUU^T\mathcal{A}UU^T \Omega)^{\dagger}(UU^T\mathcal{A}UU^T\Omega)^T\|_F\\
    = & \|U(U^T \mathcal{A} U - U^T \mathcal{A} U \widetilde{\bm{\Omega}}(\widetilde{\bm{\Omega}}^TU^T \mathcal{A} U \widetilde{\bm{\Omega}})^{\dagger}(U^T \mathcal{A} U \widetilde{\bm{\Omega}})^T )U^T\|_F\\
    = & \|U^T \mathcal{A} U - U^T \mathcal{A} U \widetilde{\bm{\Omega}}(\widetilde{\bm{\Omega}}^TU^T \mathcal{A} U \widetilde{\bm{\Omega}})^{\dagger}(U^T \mathcal{A} U \widetilde{\bm{\Omega}})^T \|_F = \|\bm{\Sigma} - \bm{\Sigma} \widetilde{\bm{\Omega}}(\widetilde{\bm{\Omega}}^T \bm{\Sigma}\widetilde{\bm{\Omega}})^{\dagger}(\bm{\Sigma}\widetilde{\bm{\Omega}})\|_F,
\end{align*}
where we used Parseval's theorem and the fact $U^T \mathcal{A} U = \bm{\Sigma}$. The remainder of the proof follows the proof of Lemma~\ref{lemma:structural_bound_nystrom}.
\end{proof}

The proofs of the expectation bounds and tailbounds are identical to the randomizxed SVD. 
\subsection{Expectation bounds}
\begin{theorem}
Let us denote
\begin{align*}
    \alpha_1 &= \frac{(p-1)k^2 + (p+1)k}{p(p-1)(p-3)} = O\left(\frac{k^2}{p^2}\right);\\
    \alpha_2 &= \frac{k(p-1) + k^2}{p(p-1)(p-3)} = O\left(\frac{kp + k^2}{p^3}\right);\\
    \alpha_3 &= \frac{2k}{p-1} = O\left(\frac{k}{p}\right);\\
    \alpha_4 &= \frac{2}{p-1} = O\left(\frac{1}{p}\right).
\end{align*}
Define
\begin{equation*}
    \beta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \delta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \xi \in \{F,*\},
\end{equation*}
and
\begin{equation*}
    \gamma_k = \frac{1}{\lambda_1 \|\bm{\widetilde{\bm{K}}}_{11}^{-1}\|_2}.
\end{equation*}
Then, if $p \geq 4$
\begin{equation*}
    \mathbb{E}\|\mathcal{A}-\widehat{\mathcal{A}}\|_F \leq \left((1 + \sqrt{\alpha_1} \frac{\beta_k^{(F)}}{\gamma_k} + \left(1+\frac{\alpha_3 + \alpha_4}{\sqrt{\alpha_1}}\right)\frac{\delta_k^{(F)}}{\gamma_k}\right) \|\bm{\Sigma}_2\|_F + \left(\sqrt{\alpha_2} \frac{\beta_k^{(*)}}{\gamma_k} + \frac{\alpha_4}{\sqrt{\alpha_2}} \frac{\delta_k^{(*)}}{\gamma_k}\right)\|\bm{\Sigma}_2\|_*,
\end{equation*}
%\begin{align*}
 %   & \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F \\
    %+& \left(\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 + (C_1+C_2)\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4 + C_1\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4 +\right.\\
    %&\left. 2 \|\widetilde{\bm{K}}_{22.1}^{1/2}\bm{\Sigma}_2 \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} + 2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \frac{\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2}{p-1} + 2\frac{\|\widetilde{\bm{K}}_{22.1}^{1/2} \bm{\Sigma}_2 \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-3/2}\|_F^2}{p-1}\right)^{1/2}
%\end{align*}
\end{theorem}
\subsection{Tailbounds}
\begin{theorem}
Let us denote
\begin{align*}
    \alpha_1 &= \frac{e^2(k+p)}{(p+1)^2};\\
    \alpha_2 & = \frac{k}{p+1};\\
    \alpha_3 & = 9 \alpha_2^2 + k \alpha_1^2;\\
    \alpha_4 & = k \alpha_1^2.
\end{align*}
Define
\begin{equation*}
    \beta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{22}\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \delta_k^{(\xi)} = \frac{\|\bm{\Sigma}_2^{1/2} \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2^{1/2}\|_{\xi}}{\lambda_1 \|\bm{\Sigma}_2\|_{\xi}}, \quad \xi \in \{2,F,*\},
\end{equation*}
and
\begin{equation*}
    \gamma_k = \frac{1}{\lambda_1 \|\bm{\widetilde{\bm{K}}}_{11}^{-1}\|_2}.
\end{equation*}
Assume that $p \geq 4$ and $u,t > 1$. Then with probability at least $1-3t^{-p}-e^{-u^2/2}$ we have
\begin{align*}
    \|\mathcal{A}-\widehat{\mathcal{A}}\|_F \leq &\|\bm{\Sigma}_2\|_F + 2 \alpha_1 t^2 u^2 \frac{\beta_k^{(2)}}{\gamma_k} \|\bm{\Sigma}_2\|_2 + 2\left( \sqrt{\alpha_3} t^2\frac{\beta_k^{(2)}}{\gamma_k} + \left(1 + \frac{6\alpha_2}{\sqrt{\alpha_3}}\right) \frac{\delta_k^{(2)}}{\gamma_k}\right)\|\bm{\Sigma}_2\|_F\\
    + & 2\left(\sqrt{\alpha_4} t^2 \frac{\beta_k^{(*)}}{\gamma_k} + \frac{4\alpha_1}{\sqrt{\alpha_4}} \frac{\delta_k^{(*)}}{\gamma_k}\right)\|\bm{\Sigma}_2\|_*
\end{align*}
%\begin{align*}
    %&\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F + \frac{2e^2(k+p)}{(p+1)^2}\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_2^2 \|\widetilde{\bm{K}}_{11}^{-1}\|_2 t^2 u^2\\
    %+ & 2\left(\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{(4)}^4 + \|\bm{\Sigma}^{1/2}_2\widetilde{\bm{K}}_{22.1}^{1/2}\|_{(4)}^4\left(\frac{9\tr(\widetilde{\bm{K}}_{11}^{-1})^2}{(p+1)^2} + \frac{e^4\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2(k+p)^2}{(p+1)^4} \right)t^4\right.\\
    %+ & \left. \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^4\frac{e^4\|\widetilde{\bm{K}}_{11}^{-1}\|_F^2(k+p)^2}{(p+1)^4}t^4+ 2 \|\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T \bm{\Sigma}_2 \widetilde{\bm{K}}_{22.1}^{1/2}\|_F^2 \frac{3\tr(\widetilde{\bm{K}}_{11}^{-1})}{p+1} t^2\right.\\
    %+ &\left. 4\|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{22.1}^{1/2}\|_{F}^2 \|\bm{\Sigma}_2^{1/2}\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\|_{F}^2 \frac{e^2(k+p)\|\widetilde{\bm{K}}_{11}^{-1}\|_2 }{(p+1)^2} t^2\right)^{1/2}
%\end{align*}
\end{theorem}

==> Notes/infdim_rsvd2.tex <==
\section{The infinite dimensional randomized SVD}
\subsection{Structural bound}
\begin{lemma}[{\cite[Theorem 2]{boulle2022learning}}]\label{lemma:infrsvdstructural}
Let $\mathcal{P}_{\mathcal{A}\Omega}$ be the orthogonal projector onto $\range(\mathcal{A}\Omega)$. Then, if $\bm{\Omega}_1$ has full row-rank we have
\begin{equation*}
    \|\mathcal{A}-\mathcal{P}_{\mathcal{A} \Omega}\mathcal{A}\|_{HS}^2 \leq \|\bm{\Sigma}_2\|_F^2 + \|\bm{\Sigma}_2 \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_F^2.
\end{equation*}
\end{lemma}

\subsection{Expectation bounds}
Prepatory lemma.
\begin{lemma}\label{lemma:frob2expectation}
For fixed matrices $\bm{B}$ and $\bm{C}$ and a standard Gaussian random matrix $\bm{\Psi}$. Then,
\begin{equation*}
    \mathbb{E} \|\bm{B}\bm{\Psi} \bm{C}\|_F^4 = 2\|\bm{A}\|_{(4)}^4 \|\bm{B}\|_{(4)}^4 + \|\bm{A}\|_{F}^4 \|\bm{B}\|_{F}^4
\end{equation*}
\end{lemma}
\begin{proof}
By the unitary invariance of Gaussian random matrices we may assume without loss of generality that $\bm{B} = \bm{\Sigma}$ and $\bm{C} = \bm{S}$ are square diagonal matrices with non-negative entries. Then, 
\begin{align*}
    \mathbb{E}\|\bm{\Sigma}\bm{\Psi} \bm{S}\|_F^4 &= \mathbb{E}\left[ \left(\sum\limits_{i=1}^m \sum\limits_{j=1} ^k \sigma_i^2 s_j^2 \psi_{ij}^2 \right)^2 \right]\\
    &= \mathbb{E}\left[\sum\limits_{(i,j)} \sigma_i^4 s_j^4 \psi_{ij}^4 + \sum\limits_{(i,j) \neq (k,\ell)} \sigma_i^2 \sigma_k^2 s_j^2 s_{\ell}^2 \omega_{ij}^2 \psi_{k\ell}^2\right]\\
    &= 3 \sum\limits_{(i,j)} \sigma_i^4 s_j^4 + \sum\limits_{(i,j) \neq (k,\ell)} \sigma_i^2 \sigma_k^2 s_j ^2s_{\ell}^2\\
    &=  2\sum\limits_{(i,j)} \sigma_i^4 s_j^4 + \left(\sum\limits_{(i,j)} \sigma_i^2 s_j^2\right)^2\\
    &= 2\|\bm{\Sigma}\|_{(4)}^4 \|\bm{S}\|_{(4)}^4 + \|\bm{\Sigma}\|_{F}^4 \|\bm{S}\|_{F}^4,
\end{align*}
as required.
\end{proof}
\begin{lemma}\label{lemma:expectationbounded}
Let $\bm{D} \in \mathbb{R}^{\infty \times \infty}$ be an infinite diagonal matrix. Then for $p \geq 4$ and $s \geq 2$ we have
\begin{equation*}
    \mathbb{E}\|\bm{D}\bm{\Omega}_2\bm{\Omega}_1^{\dagger}\|_{(s)}^2 < \infty.
\end{equation*}
\end{lemma}
\begin{proof}
Note that because $s \geq 2$ we have
\begin{equation*}
    \|\bm{D}\bm{\Omega}_2\bm{\Omega}_1^{\dagger}\|_{(s)}^2 \leq \|\bm{D}\|_2^2 \|\bm{\Omega}_2\|_{F}^2\|\bm{\Omega}_1^{\dagger}\|_F^2.
\end{equation*}
By Hölder's inequality we only need to show that $\mathbb{E}\|\bm{\Omega}_2\|_F^4 < \infty$ and $\mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_F^4 < \infty$. From Lemma~\ref{lemma:inversewishart_norm_expectation} we know $\mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_F^4 < \infty$, since $\bm{\Omega}_1$ is a matrix with columns distributed as $N(\bm{0}, \widetilde{\bm{K}}_{11})$ \cite[Lemma 1]{boulle2022learning}. Now let $\bm{\Omega}_2^{(n)}$ be the truncation of $\bm{\Omega}_2$ to the first $n$ rows. Then by the Monotone Convergence Theorem we just need to show that
\begin{equation*}
    \lim\limits_{n \rightarrow \infty} \mathbb{E}\|\bm{\Omega}_2^{(n)}\|_F^4 < \infty.
\end{equation*}
Note that the columns of $\bm{\Omega}_2^{(n)}$ are distributed as $N(0, (\widetilde{\bm{K}}_{22})_{1:n,1:n})$, where $(\widetilde{\bm{K}}_{22})_{1:n,1:n}$ is the truncation of $\widetilde{\bm{K}}_{22}$ to the first $n$ rows and columns. By Lemma~\ref{lemma:frob2expectation} we know that
\begin{equation*}
    \mathbb{E}\|\bm{\Omega}_2^{(n)}\|_F^4 = 2(k+p) \|(\widetilde{\bm{K}}_{22})_{1:n,1:n})\|_{F}^2 + (k+p)^2 \tr((\widetilde{\bm{K}}_{22})_{1:n,1:n}))^2 \leq 3(k+p)^2 \tr((\widetilde{\bm{K}}_{22})_{1:n,1:n}))^2.
\end{equation*}
Note that $\tr((\widetilde{\bm{K}}_{22})_{1:n,1:n}))^2 \leq \tr(\widetilde{\bm{K}}_{22})^2 \leq \tr(\mathcal{K})^2<\infty$, since $\mathcal{K}$ is a trace class, which concludes the proof. 

\end{proof}

\begin{lemma}\label{lemma:limits}
Let $\bm{D} \in \mathbb{R}^{\infty \times \infty}$ be an infinite diagonal matrix such that $\|\bm{D}\|_{F} \leq \infty$. Let $\bm{\Omega}_2^{(n)}$ be defined such that the first $n$ rows are equal to the first $n$ rows of $\bm{\Omega}_2$ and the remaining rows we all 0. Then, for $s \geq 2$ and $p \geq 4$ we have
\begin{equation*}
    \lim\limits_{n \rightarrow \infty} \mathbb{E}\|\bm{D}\bm{\Omega}_2^{(n)} \bm{\Omega}_1^{\dagger}\|_{(s)}^2 = \mathbb{E}\|\bm{D}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(s)}^2.
\end{equation*}
\end{lemma}
\begin{proof}
Define
\begin{equation*}
    X_n = \|\bm{D}\bm{\Omega}_2^{(n)} \bm{\Omega}_1^{\dagger}\|_{(s)}, \quad X = \|\bm{D}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(s)}.
\end{equation*}
Note that since $X \geq X_n$ almost surely we have
\begin{align*}
    &\mathbb{E}[X^2 - X_n^2] = \mathbb{E}[(X+X_n)(X-X_n)] \leq 2 \mathbb{E}[X(X-X_n)]\\
    \leq & 2\sqrt{\mathbb{E}X^2}\sqrt{\mathbb{E}[(X-X_n)^2]}.
\end{align*}
Since $\mathbb{E}X^2 < \infty$ by Lemma~\ref{lemma:expectationbounded} we must only show that $\mathbb{E}[(X-X_n)^2] \rightarrow 0$ as $n \rightarrow \infty$. By the triangle inequality, submultiplicativity, and utilizing that $s \geq 2$ we have
\begin{equation*}
    (X-X_n)^2 \leq \|\bm{D}\|_2^2 \|\bm{\Omega}_1^{\dagger}\|_F^2 \|\bm{\Omega}_2-\bm{\Omega}_2^{(n)}\|_F^2.
\end{equation*}
By Hölder's inequality it suffices to show that
\begin{equation*}
    \mathbb{E}\|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_F^4 \rightarrow 0
\end{equation*}
as $n \rightarrow 0$, since we know $\mathbb{E}\|\bm{\Omega}_2\|_F^4 < \infty$ by Lemma~\ref{lemma:inversewishart_norm_expectation}. Let $\bm{\omega}_i$ and $\bm{\omega}_i^{(n)}$ we the $n^{\text{th}}$ column of $\bm{\Omega}_2$ and $\bm{\Omega}_2^{(n)}$ respectively.% respectively and let 
%\begin{equation*}
    %\Delta^{(n)} = \|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_F, \quad \Delta_i^{(n)} = \|\bm{\omega}_i - \bm{\omega}_i^{(n)}\|_2.
%\end{equation*}
Then,
\begin{equation*}
    0 \leq \|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_F \leq \sum\limits_{i=1}^{k+p} \|\bm{\omega}_i - \bm{\omega}_i^{(n)}\|_2 \quad \text{almost surely}.
\end{equation*}
Then, by monotonicity and triangle inequality of $\mathcal{L}_p$-norms we have
\begin{align*}
    &(\mathbb{E}[ \|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_F^4])^{1/4} \leq \left(\mathbb{E}\left[\left(\sum\limits_{i=1}^{k+p} \|\bm{\omega}_i - \bm{\omega}_i^{(n)}\|_2\right)^4\right]\right)^{1/4}\leq \sum\limits_{i=1}^{k+p} \left(\mathbb{E}\left[\|\bm{\omega}_i - \bm{\omega}_i^{(n)}\|_2^4\right]\right)^{1/4}\\
    = & (k+p) \left(\mathbb{E}\left[\|\bm{\omega}_1 - \bm{\omega}_1^{(n)}\|_2^4\right]\right)^{1/4},
\end{align*}
where the final equality follows because $\|\bm{\omega}_1 - \bm{\omega}_1^{(n)}\|_2,\ldots,\|\bm{\omega}_{k+p} - \bm{\omega}_{k+p}^{(n)}\|_2$ have the same distribution. Hence, it suffices to show that
\begin{equation*}
    \lim\limits_{n \rightarrow \infty}\mathbb{E}\left[\|\bm{\omega}_1 - \bm{\omega}_1^{(n)}\|_2^4\right] = 0. 
\end{equation*}
Indeed,
\begin{align*}
    &\mathbb{E}\left[\|\bm{\omega}_1 - \bm{\omega}_1^{(n)}\|_2^4\right] = \mathbb{E}\left[\sum\limits_{i=n+1}^{\infty} (\bm{\omega}_1)_i^4 + \sum\limits_{i \neq j} (\bm{\omega}_1)_i^2 (\bm{\omega}_1)_j^2\right] = \sum\limits_{i=n+1}^{\infty} \mathbb{E}[(\bm{\omega}_1)_i^4] + \sum\limits_{i \neq j} \mathbb{E}[(\bm{\omega}_1)_i^2 (\bm{\omega}_1)_j^2] \\
    \leq & \sum\limits_{i=n+1}^{\infty} \mathbb{E}[(\bm{\omega}_1)_i^4] + \sum\limits_{i \neq j} \sqrt{\mathbb{E}[(\bm{\omega}_1)_i^4] \mathbb{E}[(\bm{\omega}_1)_j^4]} = \left(\sum\limits_{i=n+1}^{\infty} \sqrt{\mathbb{E}[(\bm{\omega}_1)_i^4]}\right)^2 = 3 \left(\sum\limits_{i=n+1}^{\infty} (\widetilde{\bm{K}}_{22})_{ii}\right)^2 \rightarrow 0,
\end{align*}
as $n \rightarrow \infty$\footnote{the final inequality comes from the fact that $(\bm{\omega}_1)_i \sim N(0,(\widetilde{\bm{K}}_{22})_{ii})$}, as required.  
\end{proof}

\begin{theorem}\label{theorem:infrsvdexpectation}
Let $\lambda_1 = \|\bm{K}\|_2 = \|\widetilde{\bm{K}}\|_2$, and
\begin{equation*}
    \beta_k = \frac{\tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22}\bm{\Sigma}_2)}{\lambda_1 \|\bm{\Sigma}_2\|_F^2}, \quad \delta_k = \frac{\tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}\bm{\Sigma}_2)}{\lambda_1 \|\bm{\Sigma}_2\|_F^2}, \quad\gamma_k = \frac{k}{\lambda_1 \tr(\widetilde{\bm{K}}_{11}^{-1})}.
\end{equation*}
If $p \geq 4$, then
\[\mathbb{E}\|\mathcal{A}-\mathcal{P}_{\mathcal{A}\Omega}\|_F^2\leq \left(1+\frac{k}{p-1}\frac{\beta_k}{\gamma_k}+k\frac{\delta_k}{\gamma_k}\right)\|\bm{\Sigma}_2\|_F^2.\]
\end{theorem}
\begin{proof}
By Lemma~\ref{lemma:limits} and Lemma~\ref{lemma:infrsvdstructural} we just need that
\begin{equation*}
     \mathbb{E}\|\bm{\Sigma}_2\bm{\Omega}_2^{(n)}\bm{\Omega}_1^{\dagger}\|_F^2 \leq \left(1+\frac{k}{p-1}\frac{\beta_k}{\gamma_k}+k\frac{\delta_k}{\gamma_k}\right)\|\bm{\Sigma}_2\|_F^2.
\end{equation*}
Note that
\begin{equation*}
    \|\bm{\Sigma}_2\bm{\Omega}_2^{(n)}\bm{\Omega}_1^{\dagger}\|_F = \|(\bm{\Sigma}_2)_{1:n, 1:n}(\bm{\Omega}_2^{(n)})_{1:n,:}\bm{\Omega}_1^{\dagger}\|_F,
\end{equation*}
and
\begin{equation*}
    \begin{bmatrix} \bm{\Omega}_1 \\ (\bm{\Omega}_2^{(n)})_{1:n,:} \end{bmatrix} \sim N\left(\bm{0}, \widetilde{\bm{K}}_{1:(k+n), 1:(k+n)}\right).
\end{equation*}
From Theorem~\ref{theorem:frobenius_expectation_bound1} we know that 
\begin{align*}
    &\mathbb{E}\|(\bm{\Sigma}_2)_{1:n, 1:n}(\bm{\Omega}_2^{(n)})_{1:n,:}\bm{\Omega}_1^{\dagger}\|_F^2 = \|(\bm{\Sigma}_2)_{1:n,1:n}(\widetilde{\bm{K}}_{21})_{1:n,:} \widetilde{\bm{K}}_{11}^{-1}\|_F^2 + \|(\bm{\Sigma}_2)_{1:n,1:n} ((\widetilde{\bm{K}}_{22.1})_{1:n,1:n})^{1/2}\|_F^2 \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}\\
    \leq & \tr((\bm{\Sigma}_2)_{1:n,1:n}(\widetilde{\bm{K}}_{21})_{1:n,:} \widetilde{\bm{K}}_{11}^{-1}(\widetilde{\bm{K}}_{21})_{1:n,:}^T(\bm{\Sigma}_2)_{1:n,1:n})\tr(\widetilde{\bm{K}}_{11}^{-1}) \\
    + & \tr((\bm{\Sigma}_2)_{1:n,1:n} (\widetilde{\bm{K}}_{22.1})_{1:n,1:n}(\bm{\Sigma}_2)_{1:n,1:n}) \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1}\\
    \leq & \tr(\bm{\Sigma}_2\widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T\bm{\Sigma}_2)\tr(\widetilde{\bm{K}}_{11}^{-1}) + \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22}\bm{\Sigma}_2) \frac{\tr(\widetilde{\bm{K}}_{11}^{-1})}{p-1} \leq \left(1+\frac{k}{p-1}\frac{\beta_k}{\gamma_k}+k\frac{\delta_k}{\gamma_k}\right)\|\bm{\Sigma}_2\|_F^2,
\end{align*}
as required. 
\end{proof}
\subsection{Tailbounds}
\begin{lemma}\label{lemma:pconvergence}
Consider the setting of Lemma~\ref{lemma:limits}. Then $\|\bm{D}\bm{\Omega}_2^{(n)}\bm{\Omega}_1^{\dagger}\|_{(s)}$ converges to $\|\bm{D}\bm{\Omega}_2\bm{\Omega}_1^{\dagger}\|_{(s)}$ in distribution. 
\end{lemma}
\begin{proof}
Utilizing $s \geq 2$ we obtain
\begin{align*}
    & 0 \leq \|\bm{D} \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(s)}-\|\bm{D} \bm{\Omega}_2^{(n)} \bm{\Omega}_1^{\dagger}\|_{(s)} \leq \|\bm{D} \bm{\Omega}_2 \bm{\Omega}_1^{\dagger}-\bm{D} \bm{\Omega}_2^{(n)} \bm{\Omega}_1^{\dagger}\|_{(s)}\\
    \leq & \|\bm{D}\|_{(s)} \|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{(s)} \|\bm{\Omega}_1^{\dagger}\|_{(s)} \leq \|\bm{D}\|_{F} \|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{F} \|\bm{\Omega}_1^{\dagger}\|_{F}.
\end{align*}
Hence, it suffices to show that $\|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{F}$ converges to $0$ in distribution, since this would imply that $\|\bm{D}\|_{F} \|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{F} \|\bm{\Omega}_1^{\dagger}\|_{F}$ converges to 0 in distribution by the product rule of random variables. Since convergence in probability implies convergence in distribution we only need to show that $\|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{F}$ converges to 0 in probability. By Markov's inequality we have for any $\varepsilon > 0$
\begin{equation*}
    \mathbb{P}\left(\|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{F} > \varepsilon \right) \leq \varepsilon^{-2}\mathbb{E}\|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{F}^2.
\end{equation*}
Thus, it suffices to show that 
\begin{equation*}
    \lim\limits_{n \rightarrow \infty} \mathbb{E}\|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{F}^2=0.
\end{equation*}
Using the notation of Lemma~\ref{lemma:limits} we have
\begin{equation*}
    \mathbb{E}\|\bm{\Omega}_2 - \bm{\Omega}_2^{(n)}\|_{F}^2 = (k+p) \mathbb{E}\|\bm{\omega}_1 - \bm{\omega}_1^{(n)}\|_2^2. 
\end{equation*}
Thus, we will show 
\begin{equation*}
    \lim\limits_{n \rightarrow \infty}\mathbb{E}\|\bm{\omega}_1 - \bm{\omega}_1^{(n)}\|_2^2= 0.
\end{equation*}
Let $f \sim GP(0,\mathcal{K})$. Then,
\begin{equation*}
    (\bm{\omega}_1)_i \sim \langle u_{i+k}, f\rangle = \sum\limits_{j=1}^{\infty} \sqrt{\lambda_j} \langle u_{i+k}, \psi_j \rangle c_j, \quad c_j \stackrel{\text{iid}}{\sim} N(0,1),
\end{equation*}
where $\psi_j$ is the $i^{\text{th}}$ eigenvector of $\mathcal{K}$. Consequently,
\begin{equation*}
    (\bm{\omega}_1)_{i} \sim N\left(0, \sum\limits_{j=1}^{\infty} \lambda_j \langle u_{i+k}, \psi_j \rangle^2\right)
\end{equation*}
It is clear that $(\bm{\omega}_1)_{i}$ has a finite variance, since $\tr(\mathcal{K}) = \sum\limits_{i=1}^{\infty} \lambda_i < \infty$ and $\langle u_{i+k}, \psi_j\rangle^2 \leq 1$. For simplicity, write $\langle u_{i+k}, \psi_j \rangle = M_{ij}$
and
\begin{equation*}
    s_i^2 = \sum\limits_{j=1}^{\infty} \lambda_j M_{ij}^2.
\end{equation*}
This implies that
\begin{equation*}
    \sum\limits_{i=1}^{\infty} s_i^2 = \sum\limits_{i=1}^{\infty} \sum\limits_{j=1}^{\infty}\lambda_j M_{ij}^2 =\sum\limits_{j=1}^{\infty} \sum\limits_{i=1}^{\infty}\lambda_j M_{i,j}^2.
\end{equation*}
Note that
\begin{equation*}
    \sum\limits_{i=1}^{\infty} M_{i,j}^2 = \sum\limits_{i=1}^{\infty} \langle u_{i+k}, \psi_j \rangle^2 = \|U_2 U_2^T\psi_j\|_{L^2}^2 \leq \|\psi_j\|_{L^2}^2 = 1,
\end{equation*}
which implies that 
\begin{equation*}
    \sum\limits_{i=1}^{\infty} s_i^2 \leq \sum\limits_{j=1}^{\infty} \lambda_j = \tr(\mathcal{K}) < \infty.
\end{equation*}
Furthermore,
\begin{equation*}
    \mathbb{E}\|\bm{\omega}_1\|_2^2 = \sum\limits_{i=1}^{\infty} \mathbb{E}(\bm{\omega}_1)_{i}^2 = \sum\limits_{i=1}^{\infty} s_i^2 < \infty.
\end{equation*}
Hence,
\begin{equation*}
    \mathbb{E}\|\bm{\omega}_1-\bm{\omega}_1^{(n)}\|_2^2 = \sum\limits_{i=n+1}^{\infty} \mathbb{E}(\bm{\omega}_1)_{i}^2= \sum\limits_{i=n+1}^{\infty} s_i^2 \rightarrow_{n \rightarrow \infty} 0,
\end{equation*}
since $\sum\limits_{i=1}^{\infty} s_i^2 < \infty$, as required.
\end{proof}
\begin{theorem}
Assume that $p \geq 4$ and $u,t >1$. Then with probability at least $1-2t^{-p} - e^{-u^2/2}$ we have
\begin{equation*}
    \|\mathcal{A}-\mathcal{P}_{\mathcal{A}\Omega}\mathcal{A}\|_F \leq \left(1 + \sqrt{t^2\frac{3k}{p+1} \frac{\beta_k}{\gamma_k} + k \frac{\delta_k}{\gamma_k}}\right)\|\bm{\Sigma}_2\|_F + ut \frac{e\sqrt{k+p}}{p+1}\|\bm{\Sigma}_2\widetilde{\bm{K}}_{22.1}^{1/2}\|_2 \sqrt{\|\widetilde{\bm{K}}_{11}^{-1}\|_2}.
\end{equation*}
\end{theorem}

\begin{proof}
From Lemma~\ref{lemma:infrsvdstructural} and the subadditivity of the square-root it suffices to show that
\begin{align*}
    X &:= \|\bm{\Sigma}_2\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_F \leq \sqrt{t^2 \frac{3\tr(\widetilde{\bm{K}}_{11}^{-1})}{p+1} \tr(\bm{\Sigma}_2 \widetilde{\bm{K}}_{22} \bm{\Sigma}_2) + \tr(\bm{\Sigma}_2\widetilde{\bm{K}}_{21}\widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T) \tr(\widetilde{\bm{K}}_{11}^{-1})}\\
    + & ut \frac{e\sqrt{k+p}}{p+1}\|\bm{\Sigma}_2\widetilde{\bm{K}}_{22.1}^{1/2}\|_2 \sqrt{\|\widetilde{\bm{K}}_{11}^{-1}\|_2} =: x,
\end{align*}
with probability at least $1-2t^{-p} - e^{-u^2/2}$. Since,
\begin{equation*}
    \begin{bmatrix} \bm{\Omega}_1 \\ (\bm{\Omega}_2^{(n)})_{1:n,:} \end{bmatrix} \sim N\left(\bm{0}, \widetilde{\bm{K}}_{1:(k+n), 1:(k+n)}\right),
\end{equation*}
we know that
\begin{align*}
    X_n &:= \|\bm{\Sigma}_2 \bm{\Omega}_2^{(n)}\bm{\Omega}_1^{\dagger}\|_F = \|(\bm{\Sigma}_2)_{1:n,1:n} (\bm{\Omega}_2)_{1:n,:}\bm{\Omega}_1^{\dagger}\|_F\\
    \leq & \sqrt{t^2 \frac{3\tr(\widetilde{\bm{K}}_{11}^{-1})}{p+1} \tr((\bm{\Sigma}_2)_{1:n,1:n} (\widetilde{\bm{K}}_{22})_{1:n,1:n} (\bm{\Sigma}_2)_{1:n,1:n}) + \tr((\bm{\Sigma}_2)_{1:n,1:n}(\widetilde{\bm{K}}_{21})_{1:n,:}\widetilde{\bm{K}}_{11}^{-1}(\widetilde{\bm{K}}_{21})_{1:n,:}^T) \tr(\widetilde{\bm{K}}_{11}^{-1})}\\
    + & ut \frac{e\sqrt{k+p}}{p+1}\|(\bm{\Sigma}_2)_{1:n,1:n}((\widetilde{\bm{K}}_{22.1})_{1:n,1:n})^{1/2}\|_2 \sqrt{\|\widetilde{\bm{K}}_{11}^{-1}\|_2} =: x_n,
\end{align*}
with probability at least $1-2t^{-p}-e^{-u^2/2}$. By Lemma~\ref{lemma:pconvergence} we know that $X_n$ converges to $X$ in probability. Furthermore, $x_n \rightarrow_{n \rightarrow \infty} x$. Hence,
\begin{equation*}
    \mathbb{P}(X < x) = \lim\limits_{n \rightarrow \infty} \mathbb{P}(X_n < x_n) \geq 1-2t^{-p}-e^{-u^2/2},
\end{equation*}
which yields the desired tailbound.
\end{proof}

==> Notes/infdim_setting.tex <==
\section{The infinite dimensional setting}
We will denote matrices, possibly of infinite size, with bold capital letters, e.g. $\bm{A}$. We will denote quasi-matrices with capital letters, e.g. $A$. We will denote operators with caligraphic capital letters, e.g $\mathcal{A}$. 

Consider an Hilbert-Schmidt operator $\mathcal{A}: L^2(D_1) \mapsto L^2(D_2)$ where $D_1, D_2 \subset \mathbb{R}^n$ with Hilbert-Schmidt decomposition
\begin{equation*}
    \mathcal{A} = \sum\limits_{i=1}^{\infty} \sigma_i u_i v_i^T = U \bm{\Sigma} V^T =  \begin{bmatrix} U_1 & U_2 \end{bmatrix} \begin{bmatrix} \bm{\Sigma}_1 & \\ & \bm{\Sigma}_2 \end{bmatrix} \begin{bmatrix} V_1^T \\ V_2^T \end{bmatrix},
\end{equation*}
where $U_1 \in \mathbb{R}^{\infty \times k}, \bm{\Sigma}_1 \in \mathbb{R}^{k \times k}$ and $V_1 \in \mathbb{R}^{\infty \times k}$. Let $\mathcal{K}$ be a Gaussian process covariance kernel (it is self-adjoint and positive definite)
\begin{equation*}
    \mathcal{K}_{xy} = K(x,y) = \sum\limits_{i=1}^{\infty} \lambda_i \psi_i(x) \psi_i(y), \quad \mathcal{K} \psi_i = \lambda_i \psi_i.
\end{equation*}
Let
\begin{equation*}
    \widetilde{\bm{K}} = V^T \mathcal{K} V = \begin{bmatrix} V_1^T \mathcal{K}V_1 & V_1^T \mathcal{K}V_2 \\ V_2^T \mathcal{K}V_1 & V_2^T \mathcal{K}V_2 \end{bmatrix} = \begin{bmatrix} \widetilde{\bm{K}}_{11} & \widetilde{\bm{K}}_{21}^T \\ \widetilde{\bm{K}}_{21} & \widetilde{\bm{K}}_{22} \end{bmatrix}.
\end{equation*}
We further assume that $\rank(\widetilde{\bm{K}}_{11}) = k$ and we denote $\widetilde{\bm{K}}_{22.1} = \widetilde{\bm{K}}_{22} - \widetilde{\bm{K}}_{21} \widetilde{\bm{K}}_{11}^{-1}\widetilde{\bm{K}}_{21}^T$. Let $\Omega \in \mathbb{R}^{\infty \times (k+p)}$ where
\begin{equation*}
    \Omega = \begin{bmatrix} \omega_1 & \cdots & \omega_{k+p} \end{bmatrix}, \omega_i \stackrel{\text{iid}}{\sim} GP(0,\mathcal{K}).
\end{equation*}
When we consider the symmetric Nyström approximation we assume that $\mathcal{A}$ is a positive trace class, i.e. $\sum\limits_{i=1}^{\infty} \sigma_i < \infty$. 

==> Notes/trash/nystrom.tex <==
\section{Standard Nyström}

\begin{lemma}\label{lemma:frob4_inverse}
\begin{equation*}
    \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_F^4 = \frac{2k}{(p-1)^2(p-3)} +  \frac{2k(k-1)}{p(p-1)^2(p-3)} + \frac{k^2}{(p-1)^2}.
\end{equation*}
\end{lemma}
\begin{proof}
Let the entries of $(\bm{\Omega}_1\bm{\Omega}_1)^{-1}$ be denoted b $x_{ij}$. Note that
\begin{align*}
    &\|\bm{\Omega}_1^{\dagger}\|_F^4 = \tr((\bm{\Omega}_1 \bm{\Omega}_1^T)^{-1})^2 = \Var(\tr((\bm{\Omega}_1 \bm{\Omega}_1^T)^{-1})) + \left(\mathbb{E}\tr((\bm{\Omega}_1 \bm{\Omega}_1^T)^{-1}) \right)^2\\
    = & \Var\left(\sum\limits_{i} x_{ii}\right) + \frac{k^2}{(p-1)^2} = \sum\limits_{i} \Var(x_{ii}) + 2 \sum\limits_{i > j} \text{Cov}(x_{ii}, x_{jj}) + \frac{k^2}{(p-1)^2}\\
    = & \frac{2k}{(p-1)^2(p-3)} +  \frac{2k(k-1)}{p(p-1)^2(p-3)} + \frac{k^2}{(p-1)^2}.
\end{align*}
\end{proof}
\begin{remark}
An equivalent way of showing this is to note that if $\bm{W}^{-1} = (\bm{\Omega}_1 \bm{\Omega}_1)^{-1}$
\begin{equation*}
    \mathbb{E}[\tr(\bm{W}^{-1})^2] = \tr(\mathbb{E}\bm{W}^{-1} \otimes \bm{W}^{-1}) = \frac{kp + k(k-1)(p-2)}{p(p-1)(p-3)} = \frac{2k + k^2(p-2)}{p(p-1)(p-3)}.
\end{equation*}
\end{remark}
\begin{lemma}\label{lemma:schatten4_inverse}
\begin{equation*}
    \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_{(4)}^4 = \frac{k^2 + k(p-1)}{p(p-1)(p-3)}.
\end{equation*}
\end{lemma}
\begin{proof}
    Let $\bm{W}^{-1} = (\bm{\Omega}_1\bm{\Omega}_1)^{-1}$. Then,
    \begin{equation*}
        \mathbb{E}\|\bm{\Omega}_1^{\dagger}\|_{(4)}^4 = \mathbb{E}\|\bm{W}^{-1}\|_F^2 = \tr(\mathbb{E}[\bm{W}^{-1}\bm{W}^{-1}]) = \frac{k^2 + k(p-1)}{p(p-1)(p-3)}.
    \end{equation*}
\end{proof}
\begin{lemma}
Let $C_1 = \frac{2k +k^2(p-2)}{p(p-1)(p-3)}$ and $C_2 = \frac{k^2 + k(p-1)}{p(p-1)(p-3)}$, then
\begin{equation*}
    \mathbb{E}\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^4 = C_2(\|\bm{\Sigma}_2\|_F^2 + \|\bm{\Sigma}_2\|_*^2) + C_1 \|\bm{\Sigma}_2\|_F^2
\end{equation*}
\end{lemma}
\begin{proof}
    First condition of $\bm{\Omega}_1$ and then use Lemma~\ref{lemma:schatten4_product}, Lemma~\ref{lemma:frob4_inverse} and \ref{lemma:schatten4_inverse}. 
\end{proof}
\begin{theorem}
\begin{equation*}
    \mathbb{E}\|\bm{A}-\widehat{\bm{A}}\|_F \leq \|\bm{\Sigma}_2\|_F + \sqrt{C_2(\|\bm{\Sigma}_2\|_F^2 + \|\bm{\Sigma}_2\|_*^2) + C_1 \|\bm{\Sigma}_2\|_F^2}
\end{equation*}
\end{theorem}
\begin{proof}
    Use the structural bound, Jensen's inequality to bound $\mathbb{E}\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^2 \leq \sqrt{\mathbb{E}\|\bm{\Sigma}_2^{1/2}\bm{\Omega}_2 \bm{\Omega}_1^{\dagger}\|_{(4)}^4}$ and the derived lemmas. 
\end{proof}
